T-PRIME: Transformer-based Protocol Identification for Machine-learning at the Edge

Spectrum sharing allows different protocols of the same standard (e.g., 802.11 family) or different standards (e.g., LTE and DVB) to coexist in overlapping frequency bands. As this paradigm continues to spread, wireless systems must also evolve to identify active transmitters and unauthorized waveforms in real time under intentional distortion of preambles, extremely low signal-to-noise ratios and challenging channel conditions. We overcome limitations of correlation-based preamble matching methods in such conditions through the design of T-PRIME: a Transformer-based machine learning approach. T-PRIME learns the structural design of transmitted frames through its attention mechanism, looking at sequence patterns that go beyond the preamble alone. The paper makes three contributions: First, it compares Transformer models and demonstrates their superiority over traditional methods and state-of-the-art neural networks. Second, it rigorously analyzes T-PRIME's real-time feasibility on DeepWave's AIR-T platform. Third, it utilizes an extensive 66 GB dataset of over-the-air (OTA) WiFi transmissions for training, which is released along with the code for community use. Results reveal nearly perfect (i.e. $>98\%$) classification accuracy under simulated scenarios, showing $100\%$ detection improvement over legacy methods in low SNR ranges, $97\%$ classification accuracy for OTA single-protocol transmissions and up to $75\%$ double-protocol classification accuracy in interference scenarios.

==> article_nocolor.tex <==

\begin{abstract}
%KRC version

%Spectrum sharing allows different protocols of the same standard (e.g., 802.11 family in 2.4GHz) or different standards (LTE and DVB in 470-862 MHz) to coexist in overlapping frequency bands. As this paradigm continues to see widespread adoption, wireless systems must also evolve to identify active transmitters and classify unauthorized waveforms in real time under intentional distortion of preambles, extreme conditions of low signal to noise ratios, spectral overlap and challenging channel conditions. This paper demonstrates the limited accuracy of correlation-based preamble matching methods under the above conditions and then mitigates them through the design of T-PRIME: a transformer-based machine learning approach. T-PRIME learns the structural design of transmitted frames through its attention mechanism, looking at sequences of patterns that go beyond the preamble alone. The paper makes three contributions: First, it compares the performance of transformer-models and demonstrates their superiority over classical preamble matching and convolutional neural networks. Second, it rigorously analyzes systems-level challenges in running transformer models in real-time by testing them on DeepWave's Artificial Intelligence Radio Transceiver (AIR-T).  Third, it utilizes an extensive over-the-air (OTA) dataset of 66 GB of different WiFi waveforms for training, which is also released along with the code for community use and replication of the work. Results reveal nearly perfect (i.e. $>98\%$) classification accuracy under simulated scenarios, with up to $100\%$ detection improvement over legacy methods in low SNR ranges, $97\%$ classification accuracy for OTA single-protocol transmissions and up to $75\%$ double-protocol classification accuracy in interference scenarios.

% Mauro - Reduced word count version (max 200 for INFOCOM)
Spectrum sharing allows different protocols of the same standard (e.g., 802.11 family) or different standards (e.g., LTE and DVB) to coexist in overlapping frequency bands. As this paradigm continues to spread, wireless systems must also evolve to identify active transmitters and unauthorized waveforms in real time under intentional distortion of preambles, extremely low signal-to-noise ratios and challenging channel conditions. We overcome limitations of correlation-based preamble matching methods in such conditions through the design of T-PRIME: a Transformer-based machine learning approach. T-PRIME learns the structural design of transmitted frames through its attention mechanism, looking at sequence patterns that go beyond the preamble alone. The paper makes three contributions: First, it compares Transformer models and demonstrates their superiority over traditional methods and state-of-the-art neural networks. Second, it rigorously analyzes T-PRIME's real-time feasibility on DeepWave's AIR-T platform. Third, it utilizes an extensive 66 GB dataset of over-the-air (OTA) WiFi transmissions for training, which is released along with the code for community use. Results reveal nearly perfect (i.e. $>98\%$) classification accuracy under simulated scenarios, showing $100\%$ detection improvement over legacy methods in low SNR ranges, $97\%$ classification accuracy for OTA single-protocol transmissions and up to $75\%$ double-protocol classification accuracy in interference scenarios.

%Older version
%As new frequency bands are released for commercial applications, the demarcation between licensed and unlicensed spectrum is becoming increasingly blurred. While this wider selection of frequencies offers potential solutions, the escalating number and diversity of wireless devices exacerbate the issue of spectrum scarcity. Consequently, the need for effective multi-protocol spectrum sharing methods becomes paramount. With their self-attention mechanism, transformers neural networks capture global dependencies and long-range interactions, enabling effective modeling of complex relationships within wireless signals. This capability makes transformers particularly well-suited for protocol classification, as they can capture the intricate patterns and characteristics that differentiate between various wireless protocols, even in the presence of noise, interference, and channel distortions. In this work we present first a comparative simulation study on the performance of transformer versus convolutional neural network (CNN) architectures for WiFi protocol classification under different channel models and noise levels. Once  transformer superiority over CNN is established, we deploy the proposed model on DeepWave's Artificial Intelligence Radio Transceiver (AIR-T) and test it with real-world over-the-air (OTA) transmissions. Our approach demonstrates a $> XX\%$ classification accuracy under simulated and OTA scenarios and an increase of $YY\%$ detection accuracy over traditional methods.
\end{abstract}

\begin{IEEEkeywords}
deep learning, protocol classification, edge computing
\end{IEEEkeywords}

\section{Introduction}
%The proliferation and the ever-increasing demand for wireless services have led to the scarcity of available spectrum resources \cite{zhang2022machine}. As a result, various wireless communication protocols coexist within the same frequency bands, leading to congested wireless spectrum environments \cite{schmidt2017wireless}. Moreover, security concerns arise when unauthorized transmissions occupy or interfere with unintended frequencies, posing risks to first responders and other critical operations \cite{jagannath2021multi}. %In such scenarios, effective protocol classification emerges as a vital mechanism for efficient spectrum management and utilization. Protocol classification entails the identification and categorization of wireless communication protocols operating within a given frequency range. 
%By detecting the diverse protocols present in a crowded spectrum, regulatory bodies, network operators, and researchers can devise intelligent strategies to mitigate interference, improve spectral efficiency, and enhance overall wireless system performance. 

The increasing demand for wireless services has caused a scarcity of spectrum resources \cite{zhang2022machine}. This results in congested wireless spectrum environments as various communication protocols coexist in the same frequency bands \cite{schmidt2017wireless}. Unauthorized transmissions further raise security concerns, posing risks to critical operations \cite{jagannath2021multi}. Detecting diverse protocols in crowded spectrums allows for intelligent strategies to mitigate interference, improve spectral efficiency, and enhance overall wireless system performance, benefiting regulatory bodies, network operators, and researchers.

\begin{figure}[t]
    \centering
    \includegraphics[width=9cm]{figures/DSTL_Overview_Infocom2024.pdf}
    \caption{T-PRIME system overview and receiver design. }
    \label{Fig: system overview}
\end{figure}

\noindent $\bullet$ \textbf{Problems with legacy methods of protocol classification.} %
Legacy methods require extensive prior knowledge of protocols, leading to challenges in detecting new protocols. %in dynamic spectrum sharing scenarios. 
Even with full protocol knowledge, correlation-based methods suffer from reduced detection accuracy in low SNR conditions and when multiple protocols overlap in frequency. To address these challenges, T-PRIME (shown in Fig. \ref{Fig: system overview}) adopts a Machine Learning (ML) based approach, performing protocol classification without requiring specific channel boundaries or symbol rates, even with overlapping signals and low SNR conditions.

Legacy protocol detection methods are integrated into the RF receiver network interface card, enabling fast preamble correlations in hardware. However, updating the system for new protocols leads to backward compatibility issues and potential detection errors in challenging wireless channels. On the other hand, software-defined radio (SDR) systems offer flexibility but introduce higher latencies due to data transfer and complexities in I/O and buffer management. This paper demonstrates that using edge devices with CPU and GPU on a system-on-a-module (SOM), along with careful software design, can overcome the these limitations and enable real-time processing for complex ML wireless applications on an SDR-based edge device.


%Legacy methods need extensive prior knowledge of protocols, including frame format, message ordering, and channel boundaries. Detecting new protocols in dynamic spectrum sharing scenarios without complete information, like channel variability and symbol rate shared between transceiver pairs, presents challenges. Even with full protocol knowledge, legacy methods relying on correlation with known preambles suffer from reduced detection accuracy, particularly in low signal-to-noise ratio (SNR) conditions. For example, our analysis in Sec.~\ref{sec:legacy_performance_simulation} shows that correlation-based methods are less effective as SNR decreases. Additionally, when two protocols coexist in overlapping frequency bands, preamble extraction becomes difficult, leading to missed detections. To address these challenges, T-PRIME (shown in Fig. \ref{Fig: system overview}) adopts an ML-based approach, performing protocol classification without requiring channel boundaries or symbol rates, even in the presence of overlapping signals and under low SNR conditions.



%Legacy methods require significant a-priori knowledge of the protocols of interest, including frame format, message ordering and the exact channel boundaries. However, in future dynamic spectrum sharing scenarios, the characteristics of new protocols may be unknown to incumbents. Detecting a new protocol without complete knowledge of channel boundaries,  channel variability, and importantly, the symbol rate that is typically shared between a transceiver pair, poses an open challenges. %While these systems work well for standards based communication, they do not do well in dynamic environments or in the presence of new signals. 
%In future AI/ML enabled wireless communications systems, it will no longer be possible to handcraft specialized feature extractors for specific signal types and properties. In this work, we design a generic approach to protocol identification that does not require any prior expert knowledge of the protocol.  
%Finally, even under full protocol knowledge, as in the case of legacy methods that typically use correlation with a known preamble embedded within transmitted frames, detection accuracy can be lowered by several factors. %Knowledge of the  exact pattern is essential to synchronization and format detection. 
%As an example that we show through quantitative metrics in this paper (Sec. \ref{sec:legacy_performance_simulation}),  correlation-based methods become increasingly ineffective as SNR decreases. As another example, when two protocols coexist in overlapping frequency bands, their individual preambles cannot be individually extracted, leading to certain missed detection. To mitigate these problems, T-PRIME, shown in Fig. \ref{Fig: system overview}, adopts a machine learning (ML) based solution that can perform protocol classification without knowledge of channel boundaries or symbol rates, with overlapping signals and under low SNR conditions. 

%It is essential to build channel-independent protocol detection methods that can accurately classify protocols without exact knowledge of the channel boundaries and in the presence of multiple overlapping signals.

%\noindent $\bullet$ \textbf{Problems with traditional hardware receivers.}
%Legacy protocol detection methods are typically integrated into the RF receiver network interface card, enabling fast preamble correlations in hardware. Updating the system for new protocols becomes challenging, as maintaining backward compatibility with legacy hardware requires redundant fields and hard-coded checks at the receiver side. This slows the adoption of new designs and may lead to detection errors, especially in challenging wireless channels and interference conditions.

%Conversely, software-defined radio (SDR) systems shift receiver processing to software in the host, offering flexibility in updating target preambles and introducing AI/ML modules into the receiver chain. However, this flexibility increases latencies due to transferring received IQ samples from the SDR front-end to the host, alongside complexities in I/O and buffer management, software dependencies, and inter-operation of compute resources between the front-end and the host.

%In this paper, we demonstrate that using edge devices that combine CPU and GPU on a system-on-a-module (SOM), along with careful software design, can overcome the limitations of traditional transceiver designs. This enables real-time processing for complex ML wireless applications, such as protocol identification, on an SDR-based edge device.

%Legacy protocol detection methods are generally built into the RF receiver network interface card. While this approach undoubtedly helps with performing fast preamble correlations in hardware, it introduces challenges in updating the system as new protocols are introduced. Therefore, to ensure backward compatibility with legacy hardware, protocol designers must rely on preamble detection techniques that require redundant fields and hard-coded checks at the receiver side. This slows adoption of new designs and can lead to errors in detection, especially in challenging wireless channels and interference conditions. 
%Conversely, protocol designers must also over-engineer in software to ensure backward compatibility with legacy hardware, such as XXXX. 

%As opposed to this, software defined radio (SDR) based systems shift most of the receiver processing to software in the host machine, which allows flexibly updating the target preambles and even introducing AI/ML modules into the receiver chain. This flexibility comes with the cost of higher latencies resulting from transferring received IQ samples from the SDR front-end to the host,  I/O and buffer management complexities, complex software dependencies and inter-operation of compute resources spread across the front-end and the host. In this paper, we show that by using edge devices that combine CPU and GPU system on a module (SOM) and careful software design, we can surpass limitations of traditional transceiver designs and achieve real time processing capabilities for complex ML wireless applications, such as protocol identification, in a SDR based edge device.   

%Such operations are typical to both cellular and local wireless network protocols, such as 802.11 and all its derivatives. While computationally inexpensive,  

\noindent $\bullet$ \textbf{Problems with WiFi protocol classification.} We showcase the potential of SDR based, ML enabled architectures by focusing on a challenging wireless scenario involving protocol classification. Specifically, we classify different 802.11 WiFi standards, including 802.11b, 802.11g, 802.11n, and 802.11ax. These  standards share similar preamble structures and can operate with the same MCS, frequency bands, channel bandwidths, and transmit power. Importantly, this classification is distinct from and more difficult than prior works \cite{zhang2022machine, schmidt2017wireless, jagannath2021multi}, which classify diverse protocols like LTE, WiFi, and Bluetooth from a candidate pool and lack a real time deployment.

%Our results demonstrate that the legacy WiFi method, based on preamble correlation, struggles under challenging conditions such as low SNR ($\le 0$ dB) due to multipath-channel effects, interference, and spectral overlap. In contrast, our ML-enabled approach, validated through simulations and experimental implementation, outperforms both the legacy WiFi method and existing state-of-the-art ML classifiers in such conditions.


%To demonstrate the potential of such RF architectures, we consider a realistic and challenging wireless scenario of protocol classification in which all protocols have 1) the same Modulation and Coding Scheme (MCS), 2) transmission power, and 3) operate with the same channel bandwidth. %{\color{red} Legacy detection systems built on energy detection or MCS modulation will fail under these scenarios}.
%For this reason, we define the problem as \textit{classification of different 802.11 WiFi standards, namely 802.11b, 802.11g, 802.11n and 802.11ax}, which not only can be configured to operate with the same MCS and frequency bands, but also share similarities in the structure of their preambles. We note that this is a different and significantly more challenging problem compared to prior works \cite{zhang2022machine, schmidt2017wireless, jagannath2021multi} classifying altogether different protocols from a candidate pool of LTE, WiFi, Bluetooth. Specifically for this problem, we show that the preamble correlation method followed by legacy WiFi suffers under challenging conditions of low SNR ($\le 0$ dB) due to the effects of multipath-channel, interference, and spectral overlap. This motivates our ML-enabled approach, which we show performs better in both simulation and with experimental implementation.
%Furthermore, we show how the proposed approach generalizes well over multiple channel realizatons and interference configurations, both in simulated and real world settings.

\noindent $\bullet$ \textbf{Proposed solution: T-PRIME.} 
% Transformers are the base of LLMs such as ChatGPT etc..
We demonstrate the effective use of Transformer neural networks \cite{NIPS2017_3f5ee243} for the above WiFi protocol classification problem. Transformers have gained significant interest in the deep learning community {\color{black} for their ability to ingest long sequences of data and efficiently correlate temporal features far from each other, which is particularly useful} for natural language processing tasks \cite{wolf-etal-2020-transformers}. However, their application to wireless communications is still in a nascent stage, with some works focusing on modulation classification \cite{9779340, zheng2022fine, hamidi2021mcformer}.
%
%Although Transformer-based models excel at processing sequential and time-dependent information, adapting them to work with IQ samples in the RF domain poses challenges. 
{\color{black} Although Transformer-based models excel at processing 1D sequential and time-dependent information, adapting them to work with 2D sequences of IQ samples is not straightforward.}
Additionally, it is crucial to evaluate ML models intended to be deployed as real-time classifiers on resource-constrained devices to understand the trade-offs between accuracy and delay.
Our contributions are as follows:
%We demonstrate how Transformer neural networks can be effectively used for the above problem of WiFi protocol classification. The Transformer architectures with attention mechanism \cite{NIPS2017_3f5ee243} have seen significant interest recently within the deep learning community. They demonstrate remarkable proficiency in natural language processing tasks~\cite{wolf-etal-2020-transformers}, although their use for wireless communications remains at a nascent stage with early works related to modulation classification ~\cite{9779340, zheng2022fine, hamidi2021mcformer}. 
%to accurately identify protocols under challenging scenario, such as overlapping interference cases and very low SNR levels (i.e. $\le 0$ dB). 
%While Transformer-based models excel at processing sequential and time-dependent information, helping them to learn the subtle features of wireless signals, adapting them to use IQ samples in the RF domain is not trivial. We must also evaluate ML models deployed as real time classifiers on resource constrained devices to understand the cost benefit tradeoffs of accuracy and delay as a function of model size.


\begin{itemize}
    \item We create, and publicly release{\color{black}\cite{tprime_github}}, a protocol classifier called T-PRIME based on Transformer architecture and compare it to both classical, preamble based processing and  ML based modulation detectors using a large data set of simulated WiFi signals. %Specifically, we show how the Transformer model operates with minimal knowledge of the protocols under study, as opposed to legacy methods.  
    %We study the impacts of Transformer model size on real time inference on an edge-device.
    
    \item We rigorously evaluate the performance of each of these protocol classification methods under various {\color{black} Single-Input-Single-Output (SISO)} wireless channel settings, including randomized channel realization, different signal-to-noise ratio (SNR) levels, and multiple channel models. In all these settings, T-PRIME outperforms state-of-the-art legacy and ML solutions available for classification of raw IQ signals.
    
    \item We implement T-PRIME on DeepWave's Artificial Intelligence Radio Transceiver (AIR-T) and evaluate performance in realistic scenarios. Drawing from this experience, we provide insights that will allow building a generic  ML-based wireless signal processing pipeline on SOM architectures that operates in near real-time using sequences of time-domain IQ samples.
   
    \item We obtain and release the first-of-its-kind dataset comprising over-the-air (OTA)  WiFi-signals for different protocol versions. This dataset includes transmissions collected in diverse environments, encompassing both single and overlapping transmission scenarios. %(e.g., with an additional interfering signal occupying either $25\%$ or $50\%$ of the intended transmitter's band).
    
\end{itemize}


\section{Related Work}

\noindent $\bullet$ \textbf{Preamble correlation Methods.}
Frame preamble usage for protocol identification and synchronization involves detecting a predefined symbol sequence at the start of a transmitted signal. %, which serves as a unique identifier for a wireless protocol. 
For example, the 802.11b long preamble consists of 128 scrambled 1s and 16 SFD marker bits, while the 802.11n preamble includes at least 9 symbols spread across all 52 OFDM sub-carriers.

Traditional signal processing techniques use energy detection and correlation \cite{9363693, terry2002ofdm}, requiring prior knowledge of the unique preamble sequences. However, they can be vulnerable to noise, interference, and channel variations. In Sec. \ref{sec:legacy_performance_simulation}, we demonstrate %through extensive simulations 
how legacy approaches fail at low SNR, while T-PRIME achieves highly accurate protocol classification under the same conditions.

%The use of the frame preamble for protocol identification and synchronization involves detecting a predefined sequence of symbols at the beginning of a transmitted signal. The  preamble serves as a unique identifier for a particular wireless protocol. For example, the 802.11b long preamble is a pattern of 128 scrambled 1s plus 16 SFD marker bits while the 802.11n preamble has at least 9 symbols spread over all 52 OFDM sub-carriers. Traditional signal processing techniques use a combination of energy detection and correlation~\cite{9363693}, which requires prior knowledge of the unique preamble sequences. %However, they often %require prior knowledge of the expected preamble sequences or templates for different protocols.  
%Moreover, they may be susceptible to noise, interference, and variations in channel conditions. Indeed, we demonstrate in Sec. \ref{sec:legacy_performance_simulation} through extensive simulations how legacy approaches fail at low SNR, while T-PRIME is able to correctly classify protocols with extremely high accuracy under the same conditions.
%Advanced techniques, including machine learning and deep learning approaches, are increasingly being employed to enhance preamble detection by leveraging the capabilities of these traditional signal processing techniques while improving robustness and adaptability in complex and dynamic wireless environments.

\noindent $\bullet$ \textbf{ML-based methods.}\label{background-ml}
Protocol classification via ML methods is still in a nascent stage. Zhang \emph{et al.} ~\cite{zhang2022machine} perform protocol detection between WiFi, LTE, and 5G signals using a multi-layer bidirectional RNN. %They utilize Matlab to generate signals, apply an AWGN channel, and capture the resulting IQ samples. 
{\color{black} They use 512 IQ pairs with a sliding window that as inputs to their RNN.} %However, they do not distinguish between different WiFi protocols. 
Similarly, Schmidt \emph{et al.} use a CNN to classify between WiFi, Bluetooth, and ZigBee signals \cite{schmidt2017wireless}. Jagannath and Jagannath  \cite{jagannath2021multi} perform both modulation classification and signal classification via CNNs by distinguishing between a wide range of different protocols including AM Radio, Bluetooth, WiFi, and IEEE 802.15.4  (Zigbee). %They use a multi-task learning model that has a shared convolutional and max-pool layer as well as task specific convolutional and fully connected layers. 
However, these approaches do not address the challenge of classifying similar protocols, such as different WiFi standards. %, making T-PRIME the first real-time 802.11 WiFi protocol classification system.

%Protocol classification is more challenging when the candidate protocols are similar in terms of modulation classes and frame structure, such as between different WiFi standards, which is not explored in prior work. Thus, T-PRIME addresses a key gap in the state-of-the-art as the first 802.11 WiFi protocol real-time classification system. 

There is a growing body of work that uses ML for the different problem of modulation classification.  These include CNN-based architectures \cite{o2016convolutional, shi2019deep, elyousseph2021deep, 8267032, gravelle2019sdr, huynh2020mcnet}, CNNs with a self-attention mechanism \cite{zhang2023amc} and RNNs \cite{8357902}. There is a smaller number of prior works that introduce Transformer based ML models for the modulation classification task. For example, Zhen \emph{et al.} create  spectrograms from IQ data and use an image Transformer \cite{zheng2022fine}. Hamidi-Rad and Jain \cite{hamidi2021mcformer} first use a CNN to transform the synthetically generated IQ samples to a 1 dimensional latent space input to the Transformer. They utilize this input CNN layer to help extract features in a location independent way because their IQ samples are not synchronized and start and stop at random locations.  Cai \emph{et al.} \cite{9779340} state that IQ data can not be directly applied to the Transformer because it represents only two sequences (I and Q) and a Transformer requires several sequences. They utilize a four step pre-processing technique that creates \say{patches} of IQ samples that are temporally close to each other. % from synthetic data sets. 
Finally, they use a linear projection embedding layer with additional sequence and positional encoding before the Transformer encoder layer. In contrast to these works that use complicated signal pre-processing and show results on offline inference only, T-PRIME shows how IQ samples can be directly provided as the input to a Transformer and performs well in realistic environments on an edge platform.
%These works are solving a fundamentally different problem than protocol detection. 
%The majority of prior modulation classification works, such as \cite{8977561, shi2019deep, elyousseph2021deep, 8267032, gravelle2019sdr, zhang2023amc, huynh2020mcnet}, use CNN or RNN based ML models for modulation classification. 

%While each of the 802.11 protocols support multiple modulation types, we specifically use 16-QAM for g, n, and ax and QPSK for b. Furthermore, the preamble for all 802.11 phy layer frames is sent using BPSK modulation. Thus, a modulation detector alone cannot distinguish between different 802.11 protocols.

%Prior work has mainly utilized CNN or ResNet-based models.
 %However, they each approach the input to the transformer in different manners. 
 %To the best of our knowledge there are no prior works that use ML to classify different 802.11 WiFi protocols.  



\section{T-PRIME Design}
%\section{T-PRIME Design and Implementation}
%\subsection{Neural network classifier}

% Opposite to the initial classifier presented, the decision was then to explore a Transformer-based architecture since this type of neural network has raised the interest in many research communities lately because of the great performance it has shown in different domains. This architecture  \cite{NIPS2017_3f5ee243} needs a sequence as the input. As our data is not naturally partitioned in tokens or words, making the parallelism with Natural Language Processing (NLP). 
%  We did that is to partition our input files in sequences, then into equally long slices and by flattening these slices we obtain our desired tokens. The way in which we flatten these is by interleaving the I and Q values as you can see in Figure \ref{Fig: IQtotokens}.

% Once we have obtain input sequence we define the final design (Figure \ref{Fig: Transformer arch}) of the Transformer architecture. The key aspect of this type of NN is the so-called attention mechanism. It allows the model to create better representations of the inputted tokens by mixing their information. The contextualized embeddings or representations after the Transformer encoder layers will be followed by a Fully-Connected layer and an Output layer with a neuron for each of the four classes in our problem. Since the task for our model is simply a classification one, we only used the encoder part of the full Transformer architecture. The final architecture also has again an initial norm layer, and the same kind of activation function, a logSoftmax.
% The hyperparameters were chosen through a hypertuning phase. Through this exploration we decided on two different values for the length of the sequence and of the tokens that gives us two different model sizes. These are the named SM transformer with 24 tokens of length 64 as the input and the LG with a sequence of 64 tokens of length 128. These two models differ in about 5.2 M params.

%\begin{figure}[t]
%    \centering
%    \includegraphics[width=0.8\linewidth]{figures/Transformer.png}
%    \caption{The general Transformer architecture with N layers can be seen on the left. The Multi-Head Attention mechanism, expanded on the right, is the key component of the Transformer.}
%    \label{Fig: Transformer overview}
%\end{figure}

%We implement two different neural network protocol classifiers, one based on a 1D CNN model and another based on transformer architecture with attention mechanism to derive insights on the cost-benefit tradeoffs between them. 

%Comparing these architectures demonstrates that transformers are better able to learn highly complex temporal dependencies compared to CNNs. 

%Transformers operate on sequences using  attention mechanisms \cite{niu2021review} with no recurrent network components. Intuitively, an attention mechanism is a neural network that produces a binary mask. This binary mask can be used to ``filter'' which neurons of a layer get to be fed-forward to the next layer. In \emph{self-attention} mechanisms, the attention network determines the mask using the input and/or previous layers themselves to construct the mask. Compared to an RNN, a Transformer applied  to sequences is able to model  arbitrary dependencies without regard to their distance in the input or output sequences, without the ``dampening'' factor inherent in RNNs across layers. Most importantly, these dependencies are malleable and  input dependent, and are learned from (and thereby adjust to) the input. 

%Transformers use attention mechanisms \cite{niu2021review}: an attention mechanism generates an activation mask, which acts as a filter to determine what information in a layer is fowarded to the next layer. In \emph{self-attention}, the attention network constructs the mask using input and/or previous layers. Unlike RNNs, Transformers can model arbitrary dependencies between sequence elements without considering their distance in the input or output sequences, while avoiding the \say{dampening} factor present in RNNs across layers. Most importantly, these dependencies in Transformers are malleable and input-dependent, adapting to and learned from the input data.


Transformers, as detailed in \cite{niu2021review}, employ attention mechanisms, or activation masks, which filter information within a layer for transmission to the subsequent layer. In \emph{self-attention}, the network generates this mask based on input and/or preceding layers. Transformers excel in modeling varied dependencies among sequence elements, independent of their positions in input or output sequences, unlike RNNs. Crucially, these adaptable dependencies in Transformers are shaped by and learned from input data. %Finally, Transformers mitigate the \say{dampening} effect found in RNNs across layers. 


\begin{figure}[t]
    \centering
    \includegraphics[width=.9\linewidth]{figures/Transformer_model.pdf}
    \caption{Transformer-based model architecture. %Parameters M, S of the input size will be different for the two model sizes. For the small architecture (SM), M=24, S=64 and for the large one (LG) M=64 and S=128.
    }
    \label{Fig: Transformer arch}
\end{figure}

The general Transformer architecture, as described by Vaswani \textit{et al.} \cite{NIPS2017_3f5ee243}, is composed of several stacked transformer layers shown in Fig.~\ref{Fig: Transformer arch}, typically forming an encoder-decoder structure. Each layer has two sub-layers: a multi-head attention mechanism and a feed-forward network. The input data, along with positional encoding, is fed into the Transformer. Next, it is passed to the multi-head attention mechanism. There are residual connections and normalizations around the two sub-layers. Implementations generally differ in where the normalization occurs and in the specific implementation of the feed-forward layer.

\begin{figure}[t]
    \centering
    \includegraphics[width=.8\linewidth]{figures/IQ_to_tokens.pdf}
    \caption{Transmission split into sequences, slices and, tokens.}
    \label{Fig: IQtotokens}
\end{figure}

\noindent $\bullet$ \textbf{Adapting Transformer for IQ Input.} The classical Transformer architecture requires a token sequence as input, typically achieved in NLP tasks through word embeddings and positional information. However, feeding IQ data to the Transformer is not straightforward, leading to complex approaches in prior work \cite{zheng2022fine, hamidi2021mcformer, 9779340}. Initially, we used spectrograms and a vision Transformer \cite{dosovitskiy2020image}, but this yielded lower performance compared to a baseline CNN \cite{o2016convolutional}.

To address this, we adopted an NLP-inspired approach of breaking the IQ samples into smaller \say{sentences} and \say{words}. Our dataset initially consists of $2 \times L$ samples, which are partitioned into sequences of dimension $2 \times N$ (sentences), then further sliced into $M$ slices of size $2 \times S$ (words). Instead of {\color{black} defining} a linear embedding for these \say{words} as in traditional NLP Transformers %we recognized that they already represent a high-dimensional embedding space. 
{\color{black} and since I and Q real values are defined in the [0,1] interval, we treat the $2S$-dimensional space defined by the set of all possible \say{words} as our embedding space.}
Thus, we simply flattened them by interleaving the I and Q samples into a vector of dimension $1 \times 2S$, eliminating the need for linear embeddings (see Fig.~\ref{Fig: IQtotokens}).


%The classical Transformer architecture requires a token sequence as an input. In NLP tasks, there are several methods to accomplish this. For example, each word in a sentence could be mapped to a specific token through a linear embedding and combined with positional information to form the input to the encoding layer. However, because IQ data is not naturally separated into words, understanding how to feed this data to the Transformer is not trivial, as seen by the variety of complex approaches taken in prior work \cite{zheng2022fine, hamidi2021mcformer, 9779340}. We initially created spectrograms from the IQ samples and used a vanilla vision Transformer, but this approach results in lower performance than the baseline CNN. 


%Ultimately, we borrowed from the NLP approach of breaking long strings of text into smaller sentances and words. Our data-set initially consists of a set of $2 \times L$ samples, where each column is a pair of I and Q samples. We partition that into sequences of dimension $2 \times N$, analogous to \say{sentences}. Then we partition that sequence into slices with dimension $2 \times S$, analogous to \say{words}. At this point traditional NLP Transformers use a linear embedding to assign words to some high dimensional vector space. Instead, recognizing that these slices already represent a pair of high dimensional vectors, we simply flatten them by inter-leaving the I and Q samples into a vector with dimension $1 \times 2S$. This eliminates the need for any linear embedding. 




%While tuning hyperparameters, we selected appropriate values for sequence length and token length, resulting in two different model sizes. The first model, named Small (SM) Transformer, utilized an input sequence of $N=24$ and tokens with a length of $S=64$. The second, Large (LG) model, employed a sequence of $N=64$ tokens with a length of $S=128$ each. The resulting number of parameters of SM and LG architectures are $1.6$M and $6.8$M, respectively.

%The classical transformer architecture \cite{NIPS2017_3f5ee243} requires a token sequence as input. Since our data is not naturally separated into tokens or words, we partition our input files (i.e. the received complex signals obtained via the onboard RF stream) into sequences of length $N$ and further divide them into  slices of size $S$. By interleaving the I and Q values in the complex signals, as shown in Figure \ref{Fig: IQtotokens}, we obtain a sequence of tokens that can be used as input to the transformer classifier. Note that while the original architecture described in \cite{NIPS2017_3f5ee243} is designed for Natural Language Processing (NLP) purposes and uses sequences of tokens from a lower dimensional text embedding, in our case, each \textit{word} is constituted by all the possible configurations I and Q in the complex series of samples of length $S$.


\noindent $\bullet$ \textbf{Transformer Architecture Design.} 
Our proposed Transformer architecture (Fig. \ref{Fig: Transformer arch}) omits positional encoding as it did not affect accuracy. Since our task is classification, we utilize only the encoder part of the Transformer. Contextualized embeddings from the encoder layers flow into a Fully-Connected layer and an Output layer representing the four classes in our classification. The architecture includes an initial normalization layer, \textit{LogSoftmax} as the final activation function and \textit{NLLLoss} as loss function.

%Our proposed Transformer architecture is shown in Figure \ref{Fig: Transformer arch}. While Transformers typically add positional encoding, we found it had no impact on our model's accuracy, so we excluded it. Since our model's task is classification, we employ only the encoder portion of a typical Transformer architecture. We feed contextualized embeddings from the Transformer encoder layers into a Fully-Connected layer and an Output layer corresponding to the four classes in our classification problem. The architecture also includes an initial normalization layer and uses \textit{LogSoftmax} as the final activation function and \textit{NLLLoss} as loss function.


%After determining the input sequence, we define the final design of our proposed Transformer architecture in Figure \ref{Fig: Transformer arch}. %The key feature of this type of neural network is the attention mechanism, which enables the model to create enhanced representations of the input tokens by combining their information. 
%The vanilla Transformer also adds positional encoding before feeding the input to the network. We studied the effect of adding a positional encoder, but found that it made no impact to the accuracy of our model so we did not use it. Since our model's task is purely classification, we utilized only the encoder part of the complete Transformer architecture. The contextualized embeddings, generated after passing through the Transformer encoder layers, are fed into a Fully-Connected layer and an Output layer containing a neuron for each of the four classes in our classification problem. Additionally, the final architecture includes an initial normalization layer, as well as \textit{LogSoftmax} as the last activation function.


%\begin{figure}[t]
%    \centering
%    \includegraphics[width=9cm]{figures/CNN.pdf}
%    \caption{Chosen convolutional neural network architecture with a Feed Forward classification head.}
%    \label{Fig: CNN arch}
%\end{figure}
%We take a systematic, two phase approach to evaluate T-PRIME. First, we genearte a large synthetic dataset to compare T-PRIME to the legacy correlation-based WiFi preamble detection algorithm, as well as ML models from prior work. After demonstrating that T-PRIME achieves superior results on synthetically generated datasets compared to these other candidate approaches, we perform an in-depth evaluation of T-PRIME on a more realistic dataset composed of over-the-air transmissions collected in different and complex RF environments. We also demonstrate the accuracy and latency of real-time inference through the implementation of T-PRIME in the AIR-T testbed.

We evaluate T-PRIME using a systematic two-phase approach. In the first phase, we generate a large synthetic dataset to compare T-PRIME with the legacy correlation-based WiFi preamble detection algorithm and ML models from prior work. T-PRIME achieves superior results on synthetically generated datasets compared to these other approaches. In the second phase, we conduct an in-depth evaluation of T-PRIME on a more realistic dataset consisting of over-the-air transmissions collected in diverse and complex RF environments. Additionally, we implement T-PRIME in the AIR-T testbed to demonstrate its accuracy and real-time inference latency.


\section{Offline Evaluation Over Synthetic Data}


\subsubsection{Dataset Description}\label{dataset description}
We used MATLAB's WLAN Waveform Generator to generate  802.11b, 802.11g, 802.11n and 802.11ax waveforms. This dataset contains baseband IQ samples according to the specifications shown in Table \ref{tab:Synthetic-Dataset}. For each protocol, we generate 2000 Physical layer Protocol Data Units (PPDU) bursts, each comprising of multiple packets carrying a 1000 bit random payload, saved into individual files. As 802.11b does not support a bandwidth/sampling rate of 20MHz,  the waveform is upsampled from 11MHz to 20MHz to ensure  waveforms have the same channel bandwidth and ensure the problem is challenging for the classifier.

\begin{table}[t]
    \centering
    \resizebox{\columnwidth}{!}{
        \begin{tabular}{|l| c c c c c |} 
            \hline
            \textbf{Standard}     & \textbf{Bandwidth} & \textbf{MCS} & \textbf{Modulation}  & \textbf{\#PPDU/burst} & \textbf{\#IQ/burst} \\ 
            \hline
            802.11b*  & 11MHz       & QPSK     & DSSS    &  1 & 18112     \\
            802.11g  & 20MHz       & 16-QAM (½ \& ¾)     & OFDM  & 4 \& 4 & 32960     \\
            802.11n & 20MHz      & 16-QAM (½ \& ¾)  & OFDM  & 5 \& 6 & 31340       \\
            802.11ax & 20MHz      & 16-QAM (½ \& ¾)  & OFDMA  & 5 \& 6 & 31640      \\
            \hline
            
        \end{tabular}
    }
    \caption{Synthetic dataset specifications. 802.11b* is upsampled from 11MHz to 20MHz for consistency with other signals.   PPDUs per burst are reported for each coding rate.}
    \label{tab:Synthetic-Dataset}
\end{table}

\subsubsection{Training Procedure}  \label{training procedure}
Once the burst signals have been generated, we use a PyTorch data generator to train our models that operates on a per-training batch basis to dynamically load into memory each file individually and simulate transmission through a channel model at an SNR level randomly chosen among the following options for (a) channel models: TGn, TGax, Rayleigh, no channel impairment; and (b)
    a random SNR level defined between -30 dB and 30 dB, applied using Additive White Gaussian Noise (AWGN).
We use a wrapper for Matlab's channel models standard compliant implementation and employ Model-B multi-path delay profile for TGn and TGax with device distance of 3m, while for Rayleigh model we use a single Non-Line Of Sight (NLOS) path with an average path gain of -3 dB and delay of 1.5e-9 seconds. %Each of the above channel and noise models can be applied at both training time, with varying randomness across epochs. Once transmissions are passed through the channel and noise simulator, they are sliced according to the model's input size and processed using its feed forward function.

Input sequences are pre-generated before training procedure for the complete set of baseband signals in the dataset. %, based on desired sequence size of each transformer model. 
Once sequence indexes are generated for each dataset burst, they are randomly shuffled and then separated into training and validation set with a split of 80\% and 20\%. When a mini-batch of sequences is generated at training time, the complete burst signal is retrieved and passed through a random channel model and AWGN. Finally, the input sequence is retrieved from the complete distorted signal and divided into slices as described in Fig. \ref{Fig: IQtotokens}. %This is because slices are not synchronized with the beginning of each packet and 
 Multi-path distortions thus impact the complete set of IQ samples in a batch on a per-sequence basis,  simulating realistic transmission. %Note that a new random channel instance is also generated at each channel application. 
 
 While dynamic signal augmentation is performed for both train and validation data, to evaluate the performance of our models in similar conditions we use an additional static test set, composed of 500 bursts for each protocol following the configuration in Table \ref{tab:Synthetic-Dataset}. Such test transmissions are pre-processed by creating multiple copies of the bursts that are passed through a random channel instance for all the considered channel models, for a total of an additional 2000 test packet bursts. Then, at test time, we create multiple sequences from each signal copy and evaluate them on discrete SNR levels ranging between -30 and 30 dB in increments of 5 dB. %We use the same training and evaluation procedure for all considered models.

%The final architecture's design, as well as the selected model and training hyperparameters, were determined through hyperparameter tuning. A grid search methodology was employed to evaluate various combinations of hyperparameters and find the optimal values. After conducting over 150 runs, we arrived at the following choices: a training duration of five epochs; a batch size of 122; and a learning rate of 2e-4.
The proposed T-PRIME design was finalized using the same training procedure above and a hyperparameters tuning phase based on a grid search on the validation set. The chosen training configuration for transformers architectures is 5 training epochs, batch size of 122 and learning rate 2e-4. We found that a stack of 2 transformer layers is optimal, along with two distinct sets of values for sequence length and slice length that provided nearly perfect results. The first model, named Small (SM) Transformer, utilized an input sequence of $M=24$ and tokens with a length of $S=64$. The second, Large (LG) model, employed a sequence of $M=64$ tokens with a length of $S=128$ each. The resulting number of parameters of SM and LG architectures are $1.6$M and $6.8$M, respectively.

\subsection{Comparison with state-of-the-art legacy and ML methods}

%ADD A DESCRIPTION OF COMPETITOR METHODS.

%\subsubsection{Comparison with Legacy Method}
\label{sec:legacy_performance_simulation}
We first show how T-PRIME approach can effectively improve the state-of-the-art over legacy approaches. Specifically, we use the same static test set described in Sec. \ref{dataset description} for a simulation study that processes each test transmission using the correlation-based procedure specified in the standard \cite{9363693}. We employ a set of multiple decoders provided by Matlab that use the legacy method to detect the following preambles formats: 
1) VHT (i.e. 802.11n), 2) HE-SU (i.e. 802.11ax), 3) Non-HT (i.e. 802.11g/b).
We then process our test transmissions through these functions for each channel model considered. %, using the same simulation parameters used while training on synthetic data. 
For each test signal, we simulate 100 transmissions over random channel instances for each channel model and SNR levels considered in our evaluation procedure described before. To report the accuracy of legacy procedures, %we compute the inverse Packet-Error-Rate (i.e. 1 - PER) 
{\color{black} we consider the inverse Packet-Detection-Rate (i.e. 1 - PDR), defined as the number of correct preamble format detection over the total number of simulated packets transmissions,} and compare it with accuracy of proposed architectures under the same statistical channel and SNR conditions. We evince from Fig. \ref{fig:synth-model-comparison} that both our T-PRIME models drastically outperform the legacy detection mechanism, achieving near-perfect detection accuracy already at SNR $= 0$ dB, while traditional methods completely fail to operate under such circumstances. This demonstrates how these models are still able to extract and learn powerful time-domain dependencies from received signals even in presence of strong noise or low reception power.
%To compare how the proposed approach performs with respect to traditional signal processing, we used the same synthetic data set described above to perform packet detection using standard procedures as specified in \cite{9363693}. 
%From Fig. \ref{fig:trans-cnn-comparison} we see that while traditional methods return Packet Error Rate (PER) close to $100\%$ and $50\%$ for SNR $= 0$ dB and $5$ dB, respectively, all proposed Transformer models achieve near-perfect detection accuracy (i.e. $100\%$ and $97\%$ for LG and SM, respectively). This clearly shows the benefits of deploying neural networks, and in particular Transformer architectures, to overcome limitations of traditional protocol detection approaches. 
%
%In fact, despite large quantities of noise and multi-path effects, these models are still able to extract and learn powerful time-domain dependencies in the input signals when exposed during training to multiple SNR and channel conditions, without using explicit knowledge of the preamble signature for each WiFi protocol.
%
%\begin{figure}
%     \centering
%     \begin{subfigure}[b]{0.211\textwidth}
%        \centering
%        \hbox{\hspace{0em} \includegraphics[width=4.1cm]{figures/traditional_detect/traditional_detection_TGn.eps}}
%
%        \caption{TGn}
%        \label{fig:traditional-tgn-sim}
%     \end{subfigure}
%     ~
%     \begin{subfigure}[b]{0.21\textwidth}
%        \centering
%        \hbox{\hspace{0em} \includegraphics[width=4.1cm]{figures/traditional_detect/traditional_detection_TGax.eps}}
%        \caption{TGax}
%    \label{fig:traditional-tgax-sim}
%     \end{subfigure}
%     ~
%     \begin{subfigure}[b]{0.21\textwidth}
%        \centering
%        \hbox{\hspace{0em} \includegraphics[width=4.1cm]{figures/traditional_detect/traditional_detection_Rayleigh.eps}}
%        \caption{Rayleigh}
%    \label{fig:traditional-rayleigh-sim}
%     \end{subfigure}
     
%    \caption{Packet Error Rate (PER) measured using traditional methods for each channel model considered in simulation. Note that 802.11g and 802.11b shares the same preamble structure so they would lead to the same performance. Each SNR value is averaged over $3000$ random channel realizations for each channel model.
%    }
%    \label{fig:PER-simulation}
%\end{figure}
%
%\subsubsection{State-of-the-art vs. Transformer Performance} 
%\textcolor{red} {ADD A DESCRIPTION OF COMPETITOR METHODS.}
%
%yarkin%
% \textcolor{cyan}{After establishing superiority of our approach over legacy methods, we compare our model to other state-of-the-art ML methods for wireless signal classification. While our problem formulation differs from modulation classification, it serves as a relevant example of architectures processing sequences of raw IQ samples for similar tasks. We compare T-PRIME against four state-of-the-art models in this domain: ResNet \cite{8267032}, AMCNet \cite{zhang2023amc}, MCformer \cite{hamidi2021mcformer}, and a 1D CNN model inspired by \cite{o2016convolutional} by exploring the optimal hyperparameter configurations of slice length, batch size, and learning rate for each of these models. \textit{CrossEntropyLoss} is used as the loss function. See \textit{Appendix} for detailed illustration of the experiments conducted.}
%
After establishing superiority of our approach over legacy methods, we compare our model to other state-of-the-art ML methods for wireless signal classification. While our problem formulation differs from modulation classification, it serves as a relevant example of architectures processing sequences of raw IQ samples for similar tasks. We compare T-PRIME against three state-of-the-art models in this domain: ResNet \cite{8267032}, AMCNet \cite{zhang2023amc}, and MCformer \cite{hamidi2021mcformer}, using \input{hyperparam_experiments_search_reference}For further comparison, we trained a 1D CNN model inspired by \cite{o2016convolutional} with a wider input size and slightly larger set of parameters. We used a common training configuration for all models with a batch size of 512, $M=1$ for input generation, \textit{CrossEntropyLoss} as the loss function, and a learning rate of 0.001 with exponential decay to 0.0001 when a plateau in the validation loss is reached. Table \ref{tab:model-size-comparison} lists all the models we compared, along with their input size and total number of parameters.


\input{simulation_results}

\begin{table}[]
    \centering

    % \begin{tabular}{|l|ll|}
    % \hline
    % \textbf{Model} &\textbf{ \# Param.} & \textbf{Input size} ($N \times S$) \\ \hline
    % T-PRIME LG & 6.8M & $64 \times 128$ \\
    % T-PRIME SM & 1.6M & $24 \times 64$ \\
    % 1D CNN \cite{o2016convolutional} & 4.1M & $1 \times 512$ \\
    % ResNet \cite{8267032} & 162K & $1 \times 1024$ \\
    % AMCNet \cite{zhang2023amc} & 462K & $1 \times 128$ \\
    % MCformer \cite{hamidi2021mcformer} & 78K & $1 \times 128$ \\ \hline
    % \end{tabular}
    \begin{tabular}{|l|ll|}
    \hline
    \textbf{Model} & \textbf{Input size} ($M \times S$) & \textbf{\# Parameters} \\ \hline
    T-PRIME LG & $64 \times 128$ & 6.8M \\
    T-PRIME SM & $24 \times 64$ & 1.6M \\
    1D CNN \cite{o2016convolutional} & $1 \times 512$ & 4.1M \\
    ResNet \cite{8267032} & $1 \times 1024$ & 162K \\
    AMCNet \cite{zhang2023amc} & $1 \times 128$ & 462K \\
    MCformer \cite{hamidi2021mcformer} & $1 \times 128$ & 78K \\ \hline
\end{tabular}
    \caption{Comparison between proposed architectures and state-of-the-art MCS classification architectures.}
    \label{tab:model-size-comparison}
\end{table}

%Once we established the superiority of our approach over legacy methods, we compare our model to other state-of-the-art machine learning methods for wireless signal classification.
%As noted in Sec. \ref{background-ml}, there is a growing body of work using ML models to perform modulation classification. While our problem formulation highlights how MCS classification alone is not enough to correctly classify transmission protocols, these models constitute the closest example of architectures used to process sequences of raw IQ samples for similar classification task. Therefore, we decide to compare the performance of T-PRIME against three state of the art models in this domain: ResNet \cite{8267032}, AMCNet \cite{zhang2023amc}, and MCformer \cite{hamidi2021mcformer} using optimal hyperparameters as reported by these works. For further comparison, we also trained a 1D CNN model inspired by \cite{o2016convolutional} with a wider input size and  slightly larger set of parameters. %We used the same training procedure described in Sec. \ref{training procedure} for all competitor models. 
%We use a common training configuration for all models using batch size of 512, $N = 1$ for input generation, \textit{CrossEntropyLoss} as loss function and learning rate of 0.001 with exponential decay to 0.0001 when a plateau in the validation loss is encountered. Table \ref{tab:model-size-comparison} lists all models we compared along with the input size and total number of parameters.



Fig. \ref{fig:tprime-competitors-caccuracy} illustrates that both T-PRIME LG and T-PRIME SM consistently outperform all other methods across the entire range of evaluated signal-to-noise ratios (SNRs). Notably, T-PRIME LG achieves a remarkable $>60$\% improvement over all other models at SNR $= -10$ dB, achieving 98\% accuracy. %Despite having fewer parameters, T-PRIME SM still outperforms all other models. 
From these experiments, two key points can be deduced: 1) T-PRIME's performance benefits from a larger parameter space, following the trend of Large-Language-Models (LLMs) that use substantial parameter capacity to learn complex relationships \cite{wei2022emergent}; 2) Our problem significantly differs from MCS classification, as the results suggest that larger amounts of temporal sequences are required to accurately identify the complex and less localized patterns in real-world wireless protocols, especially when protocols share the same MCS configurations. \input{hyperparam_experiments_results_reference}

%Fig. \ref{fig:tprime-competitors-caccuracy} shows that both T-PRIME LG and T-PRIME SM outperform all other methods for the entire range of SNRs evaluated. In particular, T-PRIME LG achieves a remarkable $>60$\% improvement over all other models at SNR $= -10$ dB, with an accuracy of 98\%. We note that even T-PRIME SM constitutes a valid candidate despite the lower amount of parameters, as it also outperforms all other models. We can conclude two important point form these experiments: 1) while it might seem trivial that a higher amount of parameters leads to better performances, T-PRIME follows current trend of Large-Language-Models (LLMs) \cite{wei2022emergent} and similarly use very large parameters space to learn complex relationship between temporal input sequences, in this case applied to specific protocol packet's structures emerging just from raw IQ samples; 2) as anticipated, we show that our problem is fundamentally different from MCS classification, as the results suggest that large amount of temporal sequences are needed in order to correctly identify the complex and less localized patterns in real-world wireless protocols or for protocols that share same MCS configurations.

%For the CNN model shown in Fig. \ref{Fig: CNN arch}, we choose a feed forward  convolutional model composed of two 1DCNN + \textit{MaxPool} layers, followed by a fully connected layer. The output class layer also uses \textit{LogSoftmax} as activation function. The chosen input size for CNN corresponds to a single slice (or token) of $S=512$ and it's arranged as a 2-channel 1D input, with I and Q values mapped onto the 2 input channels.
%Fig. \ref{fig:model-size-comparison} shows that Transformer architectures are able to ingest large quantities of temporal sequences while maintaining a relatively small number of parameters. Conversely, increasing the CNN's input size would incur a dramatic increase in parameters. Despite the lower number of parameters, the SM Transformer outperforms the proposed CNN in all observed channels and noise scenarios. %We  conclude that Transformers are overall better suited to learn the complex temporal relationship of received wireless signals. %{\color{red} This intuition will be confirmed later in Sec. \ref{?}.}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=9cm]{figures/Models size comparison.pdf}
%     \caption{Comparison of proposed neural network models size.}
%     \label{fig:model-size-comparison}
% \end{figure}



%Fig. \ref{fig:synth-model-comparison} shows the test accuracy over SNR levels for each candidate ML model, averaged over all the channels used for data generation in the simulated dataset. We see that the CNN models achieve modest accuracy even in higher SNR conditions for the most complex channel models (i.e. TGn and TGax), as detailed in Fig. \ref{fig:synth-model-comparison-bkdown}. As opposed to this, both Transformer classifiers achieve near-perfect classification accuracy for SNR $\ge 0$ dB. Due to the higher number of parameters, LG Transformer shows satisfying level of test accuracy even in lower SNR levels (i.e. $80 \%$ of average accuracy at SNR $= -15$ dB), demonstrating its ability to learn complex temporal patterns even in presence of large amount of noise.


\section{Real-Time Implementation on  AIR-T SDR}

SDR-based systems offer flexibility in the receiver chain and seamless integration with AI/ML modules. However, they can introduce higher latency due to challenges like I/O and buffer management, software dependencies, and distribution of computing resources for signal processing tasks. To explore these systems' challenges and showcase T-PRIME's real-time efficiency, we implemented it on Deepwave Digital's AIR-T model AIR7101, as shown in Fig \ref{Fig: system pic}. The AIR-T, built on NVIDIA's Jetson TX2 module, includes a CPU with 4 ARM A-57 cores, 2 ARM Denver2 cores, and a Pascal 256-core GPU with 8 GB of shared memory \cite{AIR-T}. This design resolves traditional SDR system issues by integrating resources on one platform, including SDR with FPGA, networking, periphery connections, an Ubuntu-based OS, and open source APIs.

%SDR based systems naturally support more flexible receiver chain and integrate well with AI/ML modules. However, they generally incur a cost of higher latency due to I/O and buffer management challenges, software dependency complexities, and distribution of computing resources for the signal processing tasks. In order to analyze the systems level challenges of performing machine learning for protocol detection on edge devices, and demonstrate the feasibility and real-time efficiency of T-PRIME, we implemented it on Deepwave Digital's AIR-T model AIR7101.  Fig \ref{Fig: system pic} shows T-PRIME making real time predictions in a lab environment.
%To support our goal of real time protocol detection using network edge devices, we implemented AIR-TPC on Deepwave Digital's AIR-T model AIR7101. 

\begin{figure}[tb]
    \centering
    \includegraphics[width=.75\linewidth]{figures/system_picture.png}
    \caption{T-PRIME running real-time classification in an AIR-T receiver. 802.11g protocol is shown to be correctly detected in this instance.}
    \label{Fig: system pic}
\end{figure}

%\subsection{AIR-T and Testbed Implementation}
For real-time protocol classification, low latency is crucial. Hence, we designed a pipeline (Fig. \ref{Fig: pipeline_overview}) with three primary functions running in parallel: receiver, signal processing, and ML inference. This parallelization removes concurrent dependencies and reduces prediction delay. It also allows individual function modification or improvement without affecting others. For instance, we deployed the same Transformer model using two frameworks (PyTorch and TensorRT) transparently. Each thread includes timing functions to calculate the average time for function completion. Additionally, we established two thread-safe FIFO queues, \texttt{q1} between receiver and signal processing threads, and \texttt{q2} between signal processing and ML inference threads. Below, we briefly describe each of these three threads; {\color{black} see also our code~\cite{tprime_github} for further details.}

%The AIR-T is built on top of NVIDIA's Jetson TX2 system on module consisting of a CPU with 4 ARM A-57 cores, 2 ARM Denver2 cores, and a Pascal 256-core GPU with 8 GB of shared memory \cite{AIR-T}. This SOM design resolves many of the issues of traditional software defined radio (SDR)  systems where resources are spread across different discrete devices or components. The AIR-T further includes an SDR  with integrated FPGA, networking and periphery connections, an Ubuntu-based OS and numerous open source APIs. 




%\subsubsection{Modular Processing Blocks for Real-time Inference}
%In order to achieve the goal of real time protocol classification, we must keep the latency to a minimum. To this end, we designed a pipeline, illustrated in Fig. \ref{Fig: pipeline_overview}, consisting of three primary functions that can run in parallel: receiver, signal processing, and ML inference.  Building each of these functions as separate threads provides two main advantages. First, it allows us to parallelize our flow, removing concurrent dependencies and reducing the delay between making new predictions. Second, it allows us to modify or improve specific functions individually without having to make any changes to the other functions. For example, we deployed the same Transformer model using two different frameworks, one using PyTorch and one using TensorRT (see ML Inference Thread). Switching between these frameworks can be done at run time and is completely transparent to the other functions. We included timing functions in each thread to calculate the average (mean) time it takes for the block to complete all its functions. Finally, we built two thread-safe FIFO queues, \texttt{q1} between the receiver and signal processing threads and \texttt{q2} between the signal processing and ML inference threads. We describe each of these three threads below.

\begin{figure}[tb]
    \centering
    \includegraphics[width=.95\linewidth]{figures/pipeline_overview3.png}
    \caption{T-PRIME pipeline overview showing three steps of the receiver, signal processing and ML processing modular blocks.}
    \label{Fig: pipeline_overview}
\end{figure}

\subsubsection{Receiver Thread} The main function of the receiver thread is to capture the raw OTA signals. The receiver thread defines several parameters such as sample rate (31.25 MHz), gain mode, and frequency for the AIR-T receiver using SoapySDR APIs. After initializing the SDR, it creates a data buffer to receive samples from the SDR. After these one time initialization steps are complete, the receive thread enters a continuous loop that reads the buffer, ensures it received the expected number of samples, and writes the vector of samples to \texttt{q1} if there is space available. 

\subsubsection{Signal Processing Thread} The signal processing thread's main function is to down-sample the received signal to 20 MHz and convert it to the format required by the ML inference thread. After reading the raw sample vector from \texttt{q1}, the thread converts the data type from interleaved shorts to numpy.complex64, normalized to the range of $[-1, 1]$. Then, %a low pass filter and re-sampling function 
we down-sample the signal from 31.25 MHz to 20 MHz, the standard channel bandwidth used in 802.11 WiFi protocols. Finally, the complex vector is converted into a real vector by interleaving the I and Q (real and imaginary) components, as shown in Fig. \ref{Fig: IQtotokens}. If space is available, the thread writes this vector to \texttt{q2}.

%The primary objective of this thread is to down-sample the received signal to 20 MHz and convert the data format to what is expected by the ML inference thread. After the signal processing thread reads the raw sample vector from \texttt{q1}, it converts the received sample data type from interleaved shorts to numpy.complex64 normalized to the range $[-1, 1]$. Next, we use a low pass filter and re-sampling function to down-sample the signal from 31.25 MHz to 20 MHz, the standard channel bandwidth used in 802.11 WiFi protocols. Finally, we convert this complex vector into a real vector by interleaving the I and Q (real and imaginary) components. This final step is visualized as the flattening of IQ samples in Fig. \ref{Fig: IQtotokens}. If there is space available the thread writes this vector to \texttt{q2}.

\subsubsection{ML Inference Thread} This thread is the core of our pipeline, performing the actual ML inference on the input samples. We deployed two different versions of this thread; a PyTorch version and a TensorRT version. TensorRT \cite{nvidiaQuickStart} uses techniques such as quantization, layer and tensor fusion, kernel tuning to optimize DL inference. Regardless of the optimization used, the thread follows the same process. After loading the model, it enters a continuous loop. If there is data available in \texttt{q2} it reads that into a tensor to use as the model input,  classifies, and appends the classification label to a text file.

%\noindent\textbf{Signal Power Normalization.}
To handle varying signal power caused by propagation effects, we incorporate a power normalization block in the ML inference thread. This function normalizes the total power of received signals to a nominal power of 1W.
%To deal with varying signal power introduced by propagation effects, we  add a power normalization block to the ML inference thread, before the received IQ samples are passed as input to the neural network. This function normalizes the total power of the received signals to a nominal power of $1$W. 
Given a generic discrete complex signal $\mathbf{s} \in \mathbb{C}^N$ of $N$ samples, we can obtain its normalized version $\mathbf{\hat{s}}$ as follows:
%\begin{equation}
$\mathbf{\hat{s}}={\mathbf{s}}/{\sqrt{\frac{\sum_{i=1}^N\left|s_i\right|}{N}}}$
%\end{equation}
where the denominator is the Root-Mean-Square (RMS) value of the incoming signal. This block makes our model more robust to power and SNR variations, eliminating the need to collect data samples and train our models under multiple power profiles. %However, it also amplifies noisy patterns when only background noise is observed.


\section{T-PRIME AIR-T Testbed  Evaluation}

We evaluated the performance of our T-Prime implementation through: \textit{(a)} the creation of an Over-the-Air (OTA) dataset, collected from the deployment of the testbed in five different locations, and use this dataset to conduct additional offline evaluation of T-Prime, \textit{(b)} power and latency profile characterization of our implementation, \textit{(c)} real-time, live tests of a deployment of our entire pipeline evaluating our models in a new environment. We describe each of these experiments below.

\subsection{Experimental Setup}
\subsubsection{Over-the-Air (OTA) Experiments}
\label{OTA_dataset_description} In order to evaluate the performance of our proposed approach in a real-world setting, we collect OTA transmissions in a variety of conditions, including different indoor scenarios and transmission power levels. To collect this data, we re-use the same receiver and signal processing blocks. Instead of passing the resulting vectors to the ML inference block, we write them to a file for offline training and testing.

\noindent $\bullet$ \textbf{Dataset collection.} 
We collected a large OTA dataset, providing a robust collection of real-world wireless channel conditions. Table \ref{tab:OTAdata} summarizes the environments for each collection set. Room A is a large open classroom, while rooms B and C are small lab rooms. The level of interference was assessed based on visible WiFi access points and other known transmitters in the 2.4 GHz band. The level of scatter considers the ratio of room dimensions to the space used by equipment and furniture. Each room's data was collected on two separate days (\_1 vs \_2). We also collected noise/background samples to measure the noise floor and test classifier performance when no active transmission occurred.

%We collected a large OTA dataset in three different rooms, on two different days, providing a robust collection of real-world wireless channel conditions. Table \ref{tab:OTAdata} shows a concise summary of the environment for each set of collections. Room A is a large open classroom, while rooms B and C are small lab rooms. The level of interference was based primarily on a count of visible WiFi access points using a WiFi analyzer app on a smart phone, but also considers the presence of other known transmitters in the 2.4 GHz band. The level of scatter is based on the volumetric ratio of room dimensions over the space utilized by equipment and installed furniture. For each room, data was collected on two separate days (\_1 vs \_2). The table also indicates where  noise/background samples have been collected for sake of noise floor measurements and to test the performance of our classifier when no active transmission is being performed.
% \begin{table}[htb]
%     \centering
%     \begin{tabular}{|l| c c c|} 
%         \hline
%         \textbf{DataSet}     & \textbf{Distance} & \textbf{Scatter} & \textbf{Interference}  \\ 
%         \hline
%         RM\_142\_1  & 3m       & Low     & Low           \\
%         RM\_142\_2  & 2m       & Low     & Medium        \\
%         RM\_572C\_1 & 1m       & Medium  & Medium        \\
%         RM\_572C\_2 & 1m       & Medium  & Medium        \\
%         RM\_573C\_1 & 1m       & High    & High          \\
%         RM\_573C\_2 & 1m       & High    & High          \\
%         \hline
        
%     \end{tabular}
%     \caption{OTA Dataset comparison. {\color{red} Maybe use room pictures from the slides? and include this table  as a "subfigure".}}
%     \label{tab: OTA data}
% \end{table}
\begin{table}[!t]
    \centering
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{|llll|rrrrr|}
        \hline
        \multicolumn{1}{|l|}{\textbf{Dataset}} & \multicolumn{1}{c|}{\textbf{Distance}} & \multicolumn{1}{c|}{\textbf{Scatter}} & \multicolumn{1}{c|}{\textbf{Interference}} & \multicolumn{5}{c|}{\textbf{\#Captures per protocol}} \\ \hline
        \multicolumn{1}{|l|}{} &  &  &  & \multicolumn{1}{l}{ax} & \multicolumn{1}{l}{b} & \multicolumn{1}{l}{n} & \multicolumn{1}{l}{g} & \multicolumn{1}{l|}{noise} \\ \hline
        \multicolumn{1}{|l|}{RM\_A\_1} & 3m & Low & Low & 200 & 206 & 200 & 200 & 0 \\
        \multicolumn{1}{|l|}{RM\_A\_2} & 2m & Low & Medium & 200 & 200 & 200 & 200 & 0 \\
        \multicolumn{1}{|l|}{RM\_B\_1} & 1m & Med & Medium & 73 & 200 & 200 & 200 & 0 \\
        \multicolumn{1}{|l|}{RM\_B\_2} & 1m & Med & Medium & 500 & 500 & 500 & 500 & 500 \\
        \multicolumn{1}{|l|}{RM\_C\_1} & 1m & High & High & 100 & 100 & 100 & 100 & 0 \\
        \multicolumn{1}{|l|}{RM\_C\_2} & 1m & High & High & 500 & 500 & 500 & 500 & 100 \\ \hline
\end{tabular}
    }
    \caption{OTA single-protocol datasets comparison. Each capture file contains 198080 IQ samples - approximately 10 \unit{\milli\second} duration. %{\color{red} Maybe use room pictures from the slides? and include this table  as a "subfigure".}
    }
    \label{tab:OTAdata}
\end{table}
%For each protocol, we generate a small set of standard compliant WiFi frames, composed of both preamble and random data payload in baseband. Once this signal is configured, we continuously transmit the given signal and capture it at the receiver side after it travels through the wireless medium. For all our data collections, we employ Ettus USRP X310 to transmit our baseband signals using $30$ dBm trasmission power (unless specified otherwise) and collect it with the modified T-PRIME. Both transmitter and receiver are configured to set their central frequency as $f_c = 2.442$ GHz, i.e. WiFi Channel 7. 
%Unless otherwise noted, both our training and testing phases include a power normalization pre-processing step.

For each protocol, we generated standard compliant WiFi frames, including preamble and random data payload in baseband. We continuously transmitted these signals and captured them at the receiver side after traveling through the wireless medium. Each capture is approximately 10 \unit{\milli\second} in duration. The transmitter was an Ettus USRP X310 with $30$ dBm transmission power, and both transmitter and receiver were set to a central frequency of $f_c = 2.442$ GHz, corresponding to WiFi Channel 7. In both training and testing phases, we applied  power normalization, unless otherwise specified.


\noindent $\bullet$ \textbf{Single-protocol  OTA dataset.} The above data collection results in an offline OTA dataset summarized in Table \ref{tab:OTAdata}. We split this into a training and test datasets in two ways. In our \emph{time-split}, for each day of data collection, we consider the first 80\% of  samples collected per protocol as a training set, and the remaining 20\% as a test set. In our \emph{scenario-split},  we perform a cross-validation study across all the location-specific datasets. We train our classifier on all OTA collections except one, which we use in its entirety to test the resulting model.  In both cases the test data  channel conditions are unseen during the training phase. 

\noindent $\bullet$ \textbf{Overlapping-protocol  OTA datasets.} We stress-tested T-PRIME in the presence of spectral overlaps, a scenario where traditional preamble detection techniques struggle due to frame collisions corrupting the preamble structure. In RM\_C, we collected two additional datasets with signals transmitted concurrently, overlapping at $25\%$ and $50\%$ spectral ratios. We considered six different overlapping protocol configurations (see Table \ref{tab:wifi_combinations}). The datasets differed in the observed wireless spectrum resolution, achieved by varying the receiver sampling rate and central frequency.

\begin{table}[!t]
    \centering
    \begin{tabular}{|c|c|c|}
        \hline
        \textbf{Configuration} & \textbf{Incumbent} & \textbf{Interferer} \\
        \hline
        C1 & 802.11g & 802.11n \\
        C2 & 802.11b & 802.11ax \\
        C3 & 802.11b & 802.11g \\
        C4 & 802.11b & 802.11n \\
        C5 & 802.11g & 802.11ax \\
        C6 & 802.11n & 802.11ax \\
        \hline
    \end{tabular}
    \caption{Protocols configuration for overlapping cases.}
    \label{tab:wifi_combinations}
\end{table}

Our goal was to test if our Transformer classifier could recognize both incumbent signals and the protocol of the interfering transmission using raw IQ time-domain samples. We defined two additional datasets with different receiver configurations: O1) the incumbent and receiver tuned to the same WiFi channel (WiFi Ch. 7) and sharing the same bandwidth, and O2) the receiver observing a wider bandwidth and tuned to an arbitrary frequency (2.45 GHz) to observe both overlapping signals in the frequency domain.
%
Table \ref{tab:OTA_overlap_dsinfo} summarizes the parameters used for the overlapping data collections, and Fig. \ref{fig:overlap_samples} visualizes each receiver configuration with C5 type (802.11g / 802.11ax) transmissions as an example. 

\begin{table}[!t]

    \centering
    \resizebox{\columnwidth}{!}{
        \begin{tabular}{|c|c|cccccc|} % Note the additional two 'c's in the argument of tabular
            \hline
            \textbf{Dataset} & $R$ & \textbf{$f_s^{\text{Rx}}$} & \textbf{$f_c^{\text{Rx}}$} & \textbf{$f_c^{\text{Tx1}}$}& \textbf{$f_c^{\text{Tx2}}$} & \textbf{\#Capt./Config} & \textbf{\#IQ/Capt.} \\ % Added the two new headers
            \hline
           RM\_C\_O1 & 25\% & 20 & 2.442 & 2.442 & 2.457 & 200 & 198080 \\
            RM\_C\_O1 & 50\% & 20 & 2.442 & 2.442 & 2.452 & 200 & 198080\\
            \hline
            RM\_C\_O2 & 25\% & 62.5 & 2.45 & 2.442 & 2.457 & 200 & 309500 \\
            RM\_C\_O2 & 50\% & 62.5 & 2.45 & 2.442 & 2.452 & 200 & 309500 \\
            \hline
        \end{tabular}
    }
    \caption{{\color{black} OTA overlapping dataset  parameters. $f_s^{\text{Rx}}$ (expressed in MHz) is receiver sampling rate. $f_c^{\text{Rx}}$, $f_c^{\text{Tx1}}$ and $f_c^{\text{Tx2}}$ (expressed in GHz) are receiver central frequency, central frequencies of first transmitter (incumbent) and central frequency of second transmitter, respectively.}}
    \label{tab:OTA_overlap_dsinfo}
    
\end{table}

\begin{figure}
     \centering
     \begin{subfigure}[b]{0.22\textwidth}
        \centering
        \hbox{\hspace{0em} \includegraphics[width=4.1cm]{figures/overlap/examples/DS3_2/gax_OVERLAP25_10__lines.png}}

        \caption{$f_s^{\text{Rx}} = 20$, $R = 25\%$}
        \label{fig:overlap25_gax_2}
     \end{subfigure}
     ~
     \begin{subfigure}[b]{0.22\textwidth}
        \centering
        \hbox{\hspace{0em} \includegraphics[width=4.1cm]{figures/overlap/examples/DS3_2/gax_OVERLAP50_10__lines.png}}
        \caption{$f_s^{\text{Rx}} = 20$, $R = 50\%$}
    \label{fig:overlap50_gax_2}
     \end{subfigure}
     \begin{subfigure}[b]{0.22\textwidth}
        \centering
        \hbox{\hspace{0em} \includegraphics[width=4.1cm]{figures/overlap/examples/DS3_1/gax_OVERLAP25_10__lines.png}}

        \caption{$f_s^{\text{Rx}} = 62.5$, $R = 25\%$}
        \label{fig:overlap25_gax_1}
     \end{subfigure}
     ~
     \begin{subfigure}[b]{0.22\textwidth}
        \centering
        \hbox{\hspace{0em} \includegraphics[width=4.1cm]{figures/overlap/examples/DS3_1/gax_OVERLAP50_10__lines.png}}
        \caption{$f_s^{\text{Rx}} = 62.5$, $R = 50\%$}
    \label{fig:overlap50_gax_1}
     \end{subfigure}
     
        \caption{ Example spectrograms of recorded transmissions used in the interference dataset. Samples are shown for each configurations of overlapping rate $R$ and sampling rate $f_s^{\text{Rx}}$ expressed in MHz.}
        \label{fig:overlap_samples}
\end{figure}


%We also stress-test T-PRIME in the presence of spectral overlaps. Note that traditional preamble detection techniques are not designed to operate in such conditions, as frame collisions would corrupt the preamble structure. This will introduce errors in the demodulation pipeline and can even make the transmission completely undetectable. 

%We collected two additional datasets in RM\_C, and in each of them, we have two signals transmitted concurrently with a spectrum overlapping ratio $R = \{25\%, 50\%\}$. We considered a set of 6 overlapping protocols configurations, listed in Table \ref{tab:wifi_combinations}. While the two datasets contain signals covering the same C1-6 overlap setting, they differ in the portion and resolution of the observed wireless spectrum, i.e. by varying the receiver sampling rate and central frequency. Our goal is to test if our Transformer classifier can recognize not only the incumbent signals, but also the protocol of the interfering transmission while observing incoming raw IQ time-domain samples. We defined two additional datasets considering the following scenarios: O1) when incumbent and receiver are tuned to the same WiFi channel (i.e. $f_c^{\text{Rx}} = 2.442$ GHz, i.e. WiFi Ch. 7) and share the same bandwidth, and O2) when the receiver is observing a wider bandwidth and is tuned on an arbitrary frequency (i.e. $f_c^{\text{Rx}} = 2.45$ GHz) chosen so that we can observe both overlapping signals in the frequency domain. %Note that such a case cannot be handled by traditional receivers, as the frequency selective interference would corrupt the preamble and, consequently, the detection of the whole transmission.
%Table \ref{tab:OTA_overlap_dsinfo} summarizes the parameters used for the overlapping data collections just described and Fig. \ref{fig:overlap_samples} visualize each receiver configuration, in this case using transmissions of C5 type (i.e. 802.11g / 802.11ax) as an example.
%This data collection process results in \ldots. 


We adapted our classifier from a single to multi-label output by replacing the last \textit{LogSoftMax} activation function with  \textit{Sigmoid} at each output neuron and using \textit{BCELoss} as loss function. We trained our classifier on all collected OTA transmissions, including single protocol and overlapping ones, using the \emph{time-split} method with the same 80/20 split for training/testing. %We collect over 200 file captures for each protocol and overlap ratio configuration, each file consisting of approximately 10 \unit{\milli\second} worth of complex IQ samples. 
Note that now we include  both non-overlapping and overlapping cases, and signals with different sampling rates (e.g. \_O2 datasets) in the training set. This challenging dataset forces the Transformer to learn different patterns and ultimately classify the protocols irrespective of their sampling rate. 





\subsubsection{Latency and Power Profile Experiments}
The AIR-T has 6 power profiles, providing several different combinations of CPUs enabled and various clock rates for the CPUs and GPU.
We performed a thorough analysis of all 6  configurations to understand the constraints of our system along with the benefit and cost of each option. %For each configuration, 
We used NVIDIA's JTOP utility to monitor power consumed while T-PRIME performed real-time protocol classification. 

\subsubsection{Real-Time Experiments}
We also evaluate the accuracy of T-PRIME LG in classifying OTA signals in real time. For this experiment we train T-PRIME using the entire single protocol OTA dataset (Table \ref{tab:OTAdata}). We deploy T-PRIME in two new locations, never seen during training. In both rooms, the transmitter is approximately 3m from the T-PRIME receiver. We sequentially generate and transmit each of the four 802.11 protocols in the same manner as described in Sec. \ref{OTA_dataset_description}. While continuously transmitting a given protocol, we capture 1001 live predictions made by T-PRIME. Each experiment lasts approximately 10s.

\subsection{Results}

\subsubsection{OTA Dataset Evaluation}
First, we show the performance of our classifier on OTA signals.

%While this block amplifies noisy patterns when only background noise is observed, leading to the possibility of false detections, it makes our model more robust to power and SNR variations, eliminating the need to collect data samples and train our models under multiple power profiles. 

\noindent $\bullet$ \textbf{Single-protocol results.}
 Fig. \ref{fig:LG-SM-avg-OTA} shows that both LG and SM models achieve an average classification accuracy $\ge 99\%$ on \emph{time-split} test data, with SM architecture slightly out-performing the LG one, possibly due to  \textit{overfitting} for the LG model.  Intuitively, a smaller variation of input patterns may be easier to \textit{learn} compared to randomly simulated scenarios in the synthetic dataset. 
Fig.~\ref{fig:cross-validation-OTA} shows the effect of the cross-validation on \emph{scenario-split} data. This highlights that RM\_C constitutes a more unique and challenging environment for our protocol classifier compared to other locations. %This highlights the need to expose our model to a wide variety of wireless scenarios to enable the model to generalize well. 

\begin{figure}[!t]
     \centering
     \begin{subfigure}[b]{0.22\textwidth}
        \centering
        \hbox{\hspace{0em} \includegraphics[width=4cm]{figures/avg_accuracy_singleOTA/Results_finetune_model_lg_ft.otaglobal.inf.RMSn_bckg.pdf}}

        \caption{LG model}
        \label{fig:OTA-LG-avg}
     \end{subfigure}
     ~
     \begin{subfigure}[b]{0.22\textwidth}
        \centering
        \hbox{\hspace{0em} \includegraphics[width=4cm]{figures/avg_accuracy_singleOTA/Results_finetune_sm.pt.otaglobal.inf.RMSn_bckg.pdf}}
        \caption{SM model}
    \label{fig:OTA-LG-avg}
     \end{subfigure}
     
        \caption{ WiFi protocol classification performance on the complete OTA test dataset for single transmissions.  Comparison between Large (LG) and Small (SM) Transformer models. }
        \label{fig:LG-SM-avg-OTA}
\end{figure}

%In order to assess how different channel conditions affect the signal features learned by our classifier,



%Hence, in order to train our classifier to be as general as possible, we need to expose our model to a wide variety of wireless scenarios.


\begin{figure}
     \centering
     \begin{subfigure}[b]{0.15\textwidth}
        \centering
        \hbox{\hspace{0em} \includegraphics[width=3.5cm]{figures/chann_impact/Results_finetune_model_lg_noRM_142_1_inf_RMSn_bckg_ft.RM_142_1.inf.RMSn_bckg.pdf}}
        \caption{RM\_A\_1}
        \label{fig:cv-RM_142_1}
     \end{subfigure}
     ~
      \begin{subfigure}[b]{0.15\textwidth}
        \centering
        \hbox{\hspace{0em} \includegraphics[width=3.5cm]{figures/chann_impact/Results_finetune_model_lg_noRM_142_2_inf_RMSn_bckg_ft.RM_142_2.inf.RMSn_bckg.pdf}}
        \caption{RM\_A\_2}
        \label{fig:cv-RM_142_2}
     \end{subfigure}
     ~
     \begin{subfigure}[b]{0.15\textwidth}
        \centering
        \hbox{\hspace{0em} \includegraphics[width=3.5cm]{figures/chann_impact/Results_finetune_model_lg_noRM_572C_1_inf_RMSn_bckg_ft.RM_572C_1.inf.RMSn_bckg.pdf}}
        \caption{RM\_B\_1}
        \label{fig:cv-RM_572C_1}
     \end{subfigure}
     ~
     \begin{subfigure}[b]{0.15\textwidth}
        \centering
        \hbox{\hspace{0em} \includegraphics[width=3.5cm]{figures/chann_impact/Results_finetune_model_lg_noRM_572C_2_inf_RMSn_bckg_ft.RM_572C_2.inf.RMSn_bckg.pdf}}
        \caption{RM\_B\_2}
        \label{fig:cv-RM_572C_2}
     \end{subfigure}
     ~
     \begin{subfigure}[b]{0.15\textwidth}
        \centering
        \hbox{\hspace{0em} \includegraphics[width=3.5cm]{figures/chann_impact/Results_finetune_model_lg_noRM_573C_1_inf_RMSn_bckg_ft.RM_573C_1.inf.RMSn_bckg.pdf}}
        \caption{RM\_C\_1}
        \label{fig:cv-RM_573C_1}
     \end{subfigure}
     ~
     \begin{subfigure}[b]{0.15\textwidth}
        \centering
        \hbox{\hspace{0em} \includegraphics[width=3.5cm]{figures/chann_impact/Results_finetune_model_lg_noRM_573C_2_inf_RMSn_bckg_ft.RM_573C_2.inf.RMSn_bckg.pdf}}
        \caption{RM\_C\_2}
        \label{fig:cv-RM_573C_2}
     \end{subfigure}
     ~
     
    \caption{ Cross-validation using LG classifier over the different OTA data collection instances. Each plot indicates what dataset is missing from the training set and the resulting model performance on that specific dataset at inference time. }
    \label{fig:cross-validation-OTA}
\end{figure}

\begin{figure}
     \centering
     \begin{subfigure}[b]{0.22\textwidth}
        \centering
        \hbox{\hspace{0em} \includegraphics[width=4cm]{figures/RMSimpact/noRMS/Results_finetune_model_sm_otaglobal_inf__bckg_ft.0dBs.inf._bckg.pdf}}
        \caption{W/O Power norm. }
        \label{fig:noRMS-0}
     \end{subfigure}
     ~
     \begin{subfigure}[b]{0.22\textwidth}
        \centering
        \hbox{\hspace{0em} \includegraphics[width=4cm]{figures/RMSimpact/yesRMS/Results_finetune_model_sm_otaglobal_inf_RMSn_bckg_ft.0dBs.inf.RMSn_bckg.pdf}}
        \caption{W/ Power norm.}
        \label{fig:yesRMS-0}
     \end{subfigure}
     
        \caption{Impact of power normalization for low SNR conditions, i.e. $P_{\text{Tx}} = 0$ dBm, on test data collected in RM\_C. }
        \label{fig:RMSimpact}
\end{figure}

% \begin{figure*}
%      \centering
%      \begin{subfigure}[b]{0.15\linewidth}
%         \centering
%         \hbox{\hspace{0em} \includegraphics[width=4cm]{figures/RMSimpact/noRMS/Results_finetune_model_sm_otaglobal_inf__bckg_ft.0dBs.inf._bckg.pdf}}
%         \caption{0 dBm}
%         \label{fig:noRMS-0}
%      \end{subfigure}
%      ~
%      \begin{subfigure}[b]{0.15\linewidth}
%         \centering
%         \hbox{\hspace{0em} \includegraphics[width=4cm]{figures/RMSimpact/noRMS/Results_finetune_model_sm_otaglobal_inf__bckg_ft.10dBs.inf._bckg.pdf}}
%         \caption{0 dBm}
%         \label{fig:noRMS-10}
%      \end{subfigure}
%      ~
%      \begin{subfigure}[b]{0.15\linewidth}
%         \centering
%         \hbox{\hspace{0em} \includegraphics[width=4cm]{figures/RMSimpact/noRMS/Results_finetune_model_sm_otaglobal_inf__bckg_ft.20dBs.inf._bckg.pdf}}
%         \caption{20 dBm}
%         \label{fig:noRMS-10}
%      \end{subfigure}
%      ~
%      \begin{subfigure}[b]{0.15\linewidth}
%         \centering
%         \hbox{\hspace{0em} \includegraphics[width=4cm]{figures/RMSimpact/noRMS/Results_finetune_model_sm_otaglobal_inf__bckg_ft.30dBs.inf._bckg.pdf}}
%         \caption{30 dBm}
%         \label{fig:noRMS-30}
%      \end{subfigure}
%      ~

%      \begin{subfigure}[b]{0.15\linewidth}
%         \centering
%         \hbox{\hspace{0em} \includegraphics[width=4cm]{figures/RMSimpact/yesRMS/Results_finetune_model_sm_otaglobal_inf_RMSn_bckg_ft.0dBs.inf.RMSn_bckg.pdf}}
%         \caption{0 dBm}
%         \label{fig:yesRMS-0}
%      \end{subfigure}
%      ~
%      \begin{subfigure}[b]{0.15\linewidth}
%         \centering
%         \hbox{\hspace{0em} \includegraphics[width=4cm]{figures/RMSimpact/yesRMS/Results_finetune_model_sm_otaglobal_inf_RMSn_bckg_ft.10dBs.inf.RMSn_bckg.pdf}}
%         \caption{10 dBm}
%         \label{fig:yesRMS-10}
%      \end{subfigure}
%      ~
%      \begin{subfigure}[b]{0.15\linewidth}
%         \centering
%         \hbox{\hspace{0em} \includegraphics[width=4cm]{figures/RMSimpact/yesRMS/Results_finetune_model_sm_otaglobal_inf_RMSn_bckg_ft.20dBs.inf.RMSn_bckg.pdf}}
%         \caption{20 dBm}
%         \label{fig:yesRMS-20}
%      \end{subfigure}
%      ~
%      \begin{subfigure}[b]{0.15\linewidth}
%         \centering
%         \hbox{\hspace{0em} \includegraphics[width=4cm]{figures/RMSimpact/yesRMS/Results_finetune_model_sm_otaglobal_inf_RMSn_bckg_ft.30dBs.inf.RMSn_bckg.pdf}}
%         \caption{30 dBm}
%         \label{fig:yesRMS-30}
%      \end{subfigure}
%      ~
     
%     \caption{  }
%     \label{fig:RMSimpact}
% \end{figure*}




\noindent $\bullet$ \textbf{Overlapping-protocol results.}
Table \ref{tab:OTA_overlap_avg_accuracy} shows the average test accuracy on the complete OTA test dataset and, separately, a detailed view of accuracy for each individual overlapping transmission dataset. We use three different metrics to determine the performance: 1) percent of ``exact" classifications, i.e. correctly classifying both protocols present in the received signals, 2) percent of times we correctly recognize a ``single" protocol and 3) the Area-Under-the-Curve (AUC) of the trained classifier. %Looking at results for each overlapping configuration, we see that test samples for RM\_537\_O2, i.e. the case in which a larger portion of the spectrum is observed, lead to higher ``exact" accuracy among the two overlapping configurations. 
These results show that
%, while observing the interfering signals only in the time-domain, 
our model tested on RM\_C\_O2 is still able to correctly detect at least one protocol $94.4\%$ and $93.1\%$ of times for $25\%$ and $50\%$ cases, respectively, and even able to detect both signals at the same time with $75.7\%$ and $66\%$ of accuracy for $R = 25\%$ and $R = 50\%$, respectively, which is not possible using legacy wireless hardware. 
%On the other hand, when the transceivers are tuned on the same channel and bandwidth, i.e. RM\_C\_O1, the ``exact" accuracy results slightly lowered, due to narrower bandwidth that doesn't allow observations of signals over their whole occupied spectrum. Interestingly, while comparing overlapping configurations, we observe the trend is inverted when comparing one overlapping case to the other: while in RM\_C\_O2 we observe a lower ``exact" accuracy (i.e. $66\%$) with $R = 50\%$, due to wider range of frequency selective interference, the same property seem to boost ``exact" accuracy for the RM\_C\_O1 case (i.e. $72\%$), as interference become more prominent and more spectral information becomes available. 
Finally, we note that single-protocol accuracy is nearly perfect for RM\_C\_O1 (i.e. $99.9\%$ in both overlap configurations), which suggests that incumbent signals that occupy most of the observed spectrum are correctly classified the majority of times. 

\begin{table}[!t]
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|rrrrr|}
\cline{2-6} 
& \multicolumn{5}{c|}{\textbf{Dataset}} \\
\cline{2-6} 
 & \multicolumn{1}{l|}{OTA (all)} & \multicolumn{2}{l|}{RM\_C\_O1} & \multicolumn{2}{l|}{RM\_C\_O2} \\ \cline{1-6} 
 \multicolumn{1}{|l|}{\textbf{Metric}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{$R = 25\%$} & \multicolumn{1}{l|}{$R = 50\%$} & \multicolumn{1}{l|}{$R = 25\%$} & \multicolumn{1}{l|}{$R = 50\%$} \\ \hline
\multicolumn{1}{|l|}{\% Exact (2/2)} & \multicolumn{1}{r|}{87.5} & 55.8 & \multicolumn{1}{r|}{72} & 75.7 & 66 \\ 
\multicolumn{1}{|l|}{\% Single (1/2)} & \multicolumn{1}{r|}{98.2} & 99.9 & \multicolumn{1}{r|}{99.9} & 94.4 & 93.1 \\ \cline{1-6}
\multicolumn{1}{|l|}{AUC} & \multicolumn{1}{r|}{0.98} & 0.878 & \multicolumn{1}{r|}{0.954} & 0.963 & 0.929 \\ \hline
\end{tabular}
}
\caption{Average test accuracy and AUC. Classifier is trained and tested over data covering all OTA locations, including single and overlap cases.}
    \label{tab:OTA_overlap_avg_accuracy}
\end{table}

Table \ref{tab:OTA_overlap_avg_protocol_acc} presents Precision\footnote{Precision = TP/(TP+FP); TP = True Positive; FP = False Positives.}, Recall\footnote{Recall = TP/(TP+FN); FN = False Negative.} % F1-score\footnote{f1-score = 2(Precision $\times$ Recall)/(Precision + Recall)}, 
and Support samples for each individual protocol in all receiver configurations. Precision in both RM\_C\_O1 cases shows higher scores for protocols 802.11b, 802.11g, and 802.11n, with a particular emphasis on 802.11b and 802.11g, as these protocols have more samples as incumbents than the others. Overall, the average Precision and Recall scores for all overlapping configurations and protocols are approximately 0.87 and 0.86, respectively. These results demonstrate the accuracy and completeness of positive predictions achieved by the proposed multi-protocol classifier architecture in this challenging interference scenario.

%To verify our intuition, Table \ref{tab:OTA_overlap_avg_protocol_acc} shows Precision\footnote{Precision = TP/(TP+FP); TP = True Positive; FP = False Positives.}, Recall\footnote{Recall = TP/(TP+FN); FN = False Negative.}, %f1-score\footnote{f1-score = 2(Precision $\times$ Recall)/(Precision + Recall)} 
%and number of Support samples for each individual protocol in all receiver configurations. If we look closely at Precision  in both RM\_C\_O1 cases, we notice that protocol 802.11b, 802.11g and 802.11n are the ones with higher score, with a particular bias toward 802.11b and 802.11g, i.e. the ones presenting the most number of samples as incumbents. More generally, we observe from Table \ref{tab:OTA_overlap_avg_protocol_acc} that Precision and Recall scores for all overlapping configurations and all protocols considered average to $0.87$ and $0.86$, respectively, which shows satisfying results in terms of accuracy and completeness of positive predictions for the proposed multi-protocol classifier architecture in this challenging interference scenario.







\begin{table}[t]
\resizebox{\columnwidth}{!}{
\begin{tabular}{|l|rrrrrr|}
\hline
Protocol & \multicolumn{2}{c|}{Precision} & \multicolumn{2}{c|}{Recall} & \multicolumn{2}{c|}{Support} \\ \hline
OTA (all) & \multicolumn{2}{l}{} & \multicolumn{2}{l}{} & \multicolumn{2}{l|}{} \\ \hline
802.11ax & \multicolumn{2}{c|}{0.94} & \multicolumn{2}{c|}{0.93} & \multicolumn{2}{c|}{25482} \\
802.11b & \multicolumn{2}{c|}{0.94} & \multicolumn{2}{c|}{0.98} & \multicolumn{2}{c|}{26154} \\
802.11n & \multicolumn{2}{c|}{0.9} & \multicolumn{2}{c|}{0.88} & \multicolumn{2}{c|}{26106} \\
802.11g & \multicolumn{2}{c|}{0.91} & \multicolumn{2}{c|}{0.91} & \multicolumn{2}{c|}{26106} \\ \hline
RM\_C\_O1 & \multicolumn{1}{l}{$R = 25\%$} & \multicolumn{1}{l|}{$R = 50\%$} & \multicolumn{1}{l}{$R = 25\%$} & \multicolumn{1}{l|}{$R = 50\%$} & \multicolumn{1}{l}{$R = 25\%$} & \multicolumn{1}{l|}{$R = 50\%$} \\ \hline
802.11ax & 0.72 & \multicolumn{1}{r|}{0.83} & 0.75 & \multicolumn{1}{r|}{0.86} & 2808 & 2808 \\
802.11b & 1 & \multicolumn{1}{r|}{1} & 1 & \multicolumn{1}{r|}{0.99} & 2808 & 2808 \\
802.11n & 0.77 & \multicolumn{1}{r|}{0.85} & 0.62 & \multicolumn{1}{r|}{0.83} & 2808 & 2808 \\
802.11g & 0.86 & \multicolumn{1}{r|}{0.96} & 0.78 & \multicolumn{1}{r|}{0.83} & 2808 & 2808 \\ \hline
RM\_C\_O2 & \multicolumn{1}{l}{$R = 25\%$} & \multicolumn{1}{l|}{$R = 50\%$} & \multicolumn{1}{l}{$R = 25\%$} & \multicolumn{1}{l|}{$R = 50\%$} & \multicolumn{1}{l}{$R = 25\%$} & \multicolumn{1}{l|}{$R = 50\%$} \\ \hline
802.11ax & 0.98 & \multicolumn{1}{r|}{0.97} & 0.97 & \multicolumn{1}{r|}{0.9} & 4329 & 4329 \\
802.11b & 0.82 & \multicolumn{1}{r|}{0.87} & 0.93 & \multicolumn{1}{r|}{0.96} & 4329 & 4329 \\
802.11n & 0.91 & \multicolumn{1}{r|}{0.78} & 0.8 & \multicolumn{1}{r|}{0.86} & 4329 & 4329 \\
802.11g & 0.86 & \multicolumn{1}{r|}{0.74} & 0.92 & \multicolumn{1}{r|}{0.8} & 4329 & 4329 \\ \hline
\end{tabular}
% \begin{tabular}{|lrrr|}
% \hline
% \multicolumn{1}{|l|}{\textbf{Protocol}} & \multicolumn{1}{l|}{\textbf{Precision}} & \multicolumn{1}{l|}{\textbf{Recall}} & \multicolumn{1}{l|}{\textbf{Support}} \\ \hline
% \multicolumn{1}{|l|}{OTA - all signals} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} \\ \hline
% \multicolumn{1}{|l|}{802.11ax} & 0.94 & 0.93 & 25482 \\
% \multicolumn{1}{|l|}{802.11b} & 0.94 & 0.98 & 26154 \\
% \multicolumn{1}{|l|}{802.11n} & 0.9 & 0.88 & 26106 \\
% \multicolumn{1}{|l|}{802.11g} & 0.91 & 0.91 & 26106 \\ \hline
% \multicolumn{1}{|l|}{RM\_C\_O1, $R = 25\%$} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} \\ \hline
% \multicolumn{1}{|l|}{802.11ax} & 0.72 & 0.75 & 2808 \\
% \multicolumn{1}{|l|}{802.11b} & 1 & 1 & 2808 \\
% \multicolumn{1}{|l|}{802.11n} & 0.77 & 0.62 & 2808 \\
% \multicolumn{1}{|l|}{802.11g} & 0.86 & 0.78 & 2808 \\ \hline
% \multicolumn{1}{|l|}{RM\_C\_O1, $R = 50\%$} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} \\ \hline
% \multicolumn{1}{|l|}{802.11ax} & 0.83 & 0.86 & 2808 \\
% \multicolumn{1}{|l|}{802.11b} & 1 & 0.99 & 2808 \\
% \multicolumn{1}{|l|}{802.11n} & 0.85 & 0.83 & 2808 \\
% \multicolumn{1}{|l|}{802.11g} & 0.96 & 0.83 & 2808 \\ \hline
% \multicolumn{1}{|l|}{RM\_C\_O2, $R = 25\%$} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} \\ \hline
% \multicolumn{1}{|l|}{802.11ax} & 0.98 & 0.97 & 4329 \\
% \multicolumn{1}{|l|}{802.11b} & 0.82 & 0.93 & 4329 \\
% \multicolumn{1}{|l|}{802.11n} & 0.91 & 0.8 & 4329 \\
% \multicolumn{1}{|l|}{802.11g} & 0.86 & 0.92 & 4329 \\ \hline
% \multicolumn{1}{|l|}{RM\_C\_O2, $R = 50\%$} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} \\ \hline
% \multicolumn{1}{|l|}{802.11ax} & 0.97 & 0.9 & 4329 \\
% \multicolumn{1}{|l|}{802.11b} & 0.87 & 0.96 & 4329 \\
% \multicolumn{1}{|l|}{802.11n} & 0.78 & 0.86 & 4329 \\
% \multicolumn{1}{|l|}{802.11g} & 0.74 & 0.8 & 4329 \\ \hline
% \end{tabular}

%     \begin{tabular}{|lrrrr|}
% \hline
% \multicolumn{1}{|l|}{\textbf{Protocol}} & \multicolumn{1}{l|}{\textbf{Precision}} & \multicolumn{1}{l|}{\textbf{Recall}} & \multicolumn{1}{l|}{\textbf{f1-score}} & \multicolumn{1}{l|}{\textbf{Support}} \\ \hline
% \multicolumn{1}{|l|}{OTA - all signals} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} \\ \hline
% \multicolumn{1}{|l|}{802.11ax} & 0.94 & 0.93 & 0.93 & 25482 \\
% \multicolumn{1}{|l|}{802.11b} & 0.94 & 0.98 & 0.96 & 26154 \\
% \multicolumn{1}{|l|}{802.11n} & 0.9 & 0.88 & 0.89 & 26106 \\
% \multicolumn{1}{|l|}{802.11g} & 0.91 & 0.91 & 0.91 & 26106 \\ \hline
% \multicolumn{1}{|l|}{RM\_537C\_O1, $R = 25\%$} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} \\ \hline
% \multicolumn{1}{|l|}{802.11ax} & 0.72 & 0.75 & 0.73 & 2808 \\
% \multicolumn{1}{|l|}{802.11b} & 1 & 1 & 1 & 2808 \\
% \multicolumn{1}{|l|}{802.11n} & 0.77 & 0.62 & 0.69 & 2808 \\
% \multicolumn{1}{|l|}{802.11g} & 0.86 & 0.78 & 0.82 & 2808 \\ \hline
% \multicolumn{1}{|l|}{RM\_537C\_O1, $R = 50\%$} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} \\ \hline
% \multicolumn{1}{|l|}{802.11ax} & 0.83 & 0.86 & 0.84 & 2808 \\
% \multicolumn{1}{|l|}{802.11b} & 1 & 0.99 & 0.99 & 2808 \\
% \multicolumn{1}{|l|}{802.11n} & 0.85 & 0.83 & 0.84 & 2808 \\
% \multicolumn{1}{|l|}{802.11g} & 0.96 & 0.83 & 0.89 & 2808 \\ \hline
% \multicolumn{1}{|l|}{RM\_537\_O2, $R = 25\%$} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} \\ \hline
% \multicolumn{1}{|l|}{802.11ax} & 0.98 & 0.97 & 0.97 & 4329 \\
% \multicolumn{1}{|l|}{802.11b} & 0.82 & 0.93 & 0.87 & 4329 \\
% \multicolumn{1}{|l|}{802.11n} & 0.91 & 0.8 & 0.85 & 4329 \\
% \multicolumn{1}{|l|}{802.11g} & 0.86 & 0.92 & 0.89 & 4329 \\ \hline
% \multicolumn{1}{|l|}{RM\_537\_O2, $R = 50\%$} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} \\ \hline
% \multicolumn{1}{|l|}{802.11ax} & 0.97 & 0.9 & 0.93 & 4329 \\
% \multicolumn{1}{|l|}{802.11b} & 0.87 & 0.96 & 0.91 & 4329 \\
% \multicolumn{1}{|l|}{802.11n} & 0.78 & 0.86 & 0.82 & 4329 \\
% \multicolumn{1}{|l|}{802.11g} & 0.74 & 0.8 & 0.77 & 4329 \\ \hline
% \end{tabular}
}
\caption{Test accuracy for individual protocols in single and overlapping transmissions. Classifier is trained and tested over data covering all OTA locations, including single and overlap cases.}
    \label{tab:OTA_overlap_avg_protocol_acc}

\end{table}

\noindent $\bullet$ \textbf{Impact of power normalization.}
We also study the impact of power normalization on an additional set of data collected under different transmission powers. Specifically, for this experiment we train our model on data collected from all locations (see Table \ref{tab:OTAdata}) but we test it on a completely different set of samples collected in RM\_C with transmissions performed at power $P_{\text{Tx}} = \{30, 20, 10, 0\}$ dBm respectively. Table \ref{tab:RMSimpact-accuracy} shows the average accuracy for each of the power profiles when power normalization is applied. While the average accuracy is consistently improved for all protocols, the most significant boost in performance is on the lower SNR end, reaching a staggering $40.3\%$ performance improvement at $P_{\text{Tx}} = 0$ dBm without the need to include any additional power variation samples in the dataset. 

\begin{table}[!t]
    \centering
    \begin{tabular}{|l| c c |}
        \hline
        $P_{\text{Tx}}$ (dBm) & \textbf{W/O Power Norm.} & \textbf{W/ Power Norm.} \\
        \hline
        0 & 52.5 & 92.8 \\
        10 & 93.8 & 95.9 \\
        20 & 93.9 & 95.3 \\
        30 & 97.3 & 97.6 \\
        \hline
    \end{tabular}
    \caption{Average test accuracy (\%) on multiple power profiles with and without signal power normalization.}
    \label{tab:RMSimpact-accuracy}
\end{table}





\subsubsection{Real-Time Latency and Power Results}

Building a pipeline with modular processing blocks that can operate in parallel is one of the keys to deploying a real-time classification system on an edge device. For example, as seen in Table \ref{tab: pipeline performance}, when using TensorRT, the Signal processing and ML inference blocks take nearly the same amount of time to process a sample. However, our pipeline allows for these processes to run in parallel producing a prediction every 10.9 \unit{\milli\second} - equivalent to 92 predictions per second.  
%
Table \ref{tab: pipeline performance} shows the power consumption and time to complete each block for all power profiles except 4-MAXP CORE DENVER which failed to run our pipeline. The top performance and most efficient power profiles from our testing are in bold. There is a clear trade off between higher performance in terms of predictions per second and higher power usage. For all power profiles, TensorRT provides better performance and is more efficient. 

% \begin{table}[tb]
% \resizebox{\columnwidth}{!}{
%     \centering
% \begin{tblr}{
%   column{even} = {c},
%   column{2} = {Silver},
%   column{3} = {Silver,c},
%   column{5} = {c},
%   cell{1}{2} = {c=2}{},
%   cell{1}{4} = {c=2}{},
%   cell{4}{2} = {c=4}{SurfCrest},
%   cell{10}{2} = {c=4}{SurfCrest},
%   vline{2-3,5} = {1}{},
%   vline{2,4,6} = {-}{},
%   vline{3,5} = {2-3,5-9,11-13}{dashed},
%   vline{2-3} = {4,10}{},
%   vline{1-2,4,6} = {5-9,11-13}{},
%   hline{1} = {2-6}{0.08em},
%   hline{4} = {2-5}{},
%   hline{5,11} = {-}{},
%   hline{10} = {1-5}{},
%   hline{14} = {-}{0.08em}
% }
%             & \textbf{Pytorch}                     &                                    & \textbf{TensorRT}                    &                                    \\
%             & {\textbf{Lowest Latency}} & {\textit{Lowest Power}} & {\textbf{Lowest Latency}} & {\textit{Lowest Power}} \\
%             & 0-MAXN                               & 1-MAXQ                             & 5-MAXN ARM                           & 1-MAXQ                             \\
%             & Average Power Consumption (mW)       &                                    &                                      &                                    \\
% CPU         & 1551                                 & 704                                & 1540                                 & \textit{672}                       \\
% DDR         & 1595                                 & 842                                & 997                                  & \textit{780}                       \\
% GPU         & 1074                                 & 486                                & 578                                  & \textit{264}                       \\
% SOC         & 1000                                 & 625                                & 628                                  & \textit{598}                       \\
% All         & 6933                                 & 4283                               & 5426                                 & \textit{3923}                      \\
%             & Average Latency Time (ms)            &                                    &                                      &                                    \\
% Receiver    & \textbf{0.4105}                      & 0.7252                             & 0.5054                               & 0.6162                             \\
% Signal Pro. & 9.843                                & 15.39                              & \textbf{9.620}                       & 15.45                              \\
% ML Inf.     & 18.98                                & 29.18                              & \textbf{10.86}                       & 15.91                              
% \end{tblr}
% }
% \caption{Highlight of T-PRIME pipeline performance for each block showing the \textbf{lowest latency} and \emph{lowest power} using different power profiles and ML inference optimization. The optimized TensorRT gives the fastest and most power efficient results without compromising ML inference accuracy. }
% \label{tab: pipeline performance}
% \end{table}


\begin{table}
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{|l|c|c|c|c|c|} 
\hline
 & 0-MAXN & 1-MAXQ & 2-MAXP & 3-MAXP & 5-MAXN \\
 & ALL &  & ALL & ARM & ARM \\ 
\hline
\multicolumn{6}{|c|}{{\cellcolor[rgb]{0.753,0.753,0.753}}PyTorch} \\
\multicolumn{6}{|c|}{{\cellcolor[rgb]{0.753,0.753,0.753}}Average Power Consumption (\unit{\milli\watt})} \\ 
\hline
\rowcolor[rgb]{0.753,0.753,0.753} CPU & 1551 & 704 & 807 & 1457 & 1472 \\
\rowcolor[rgb]{0.753,0.753,0.753} DDR & 1595 & 842 & 900 & 999 & 1007 \\
\rowcolor[rgb]{0.753,0.753,0.753} GPU & 1074 & 486 & 366 & 434 & 435 \\
\rowcolor[rgb]{0.753,0.753,0.753} SOC & 1000 & 625 & 625 & 627 & 628 \\
\rowcolor[rgb]{0.753,0.753,0.753} ALL & 6933 & 4283 & 4338 & 5195 & 5242 \\ 
\hline
\multicolumn{6}{|c|}{{\cellcolor[rgb]{0.753,0.753,0.753}}Average Latency Time (\unit{\milli\second})} \\ 
\hline
\rowcolor[rgb]{0.753,0.753,0.753} Reciever & 0.4105 & 0.7252 & 0.44307 & \textbf{0.4103} & 0.4105 \\
\rowcolor[rgb]{0.753,0.753,0.753} Signal Pro. & 9.843 & 15.39 & 14.68 & 10.49 & 10.46 \\
\rowcolor[rgb]{0.753,0.753,0.753} ML Thread & 18.98 & 29.18 & 29.58 & 22.28 & 22.27 \\ 
\hhline{|======|}
\multicolumn{6}{|c|}{\textit{\textbf{TensorRT}}} \\
\multicolumn{6}{|c|}{Average Power Consumption (\unit{\milli\watt})} \\ 
\hline
CPU & 1579 & \textit{672} & 825 & 1515 & 1540 \\
DDR & 904 & \textit{780} & 958 & 1131 & 997 \\
GPU & 404 & \textit{264} & 436 & 629 & 578 \\
SOC & 610 & \textit{598} & 617 & 668 & 628 \\
ALL & 5170 & \textit{3923} & 4505 & 5668 & 5426 \\ 
\hline
\multicolumn{6}{|c|}{Average Latency Time (\unit{\milli\second})} \\ 
\hline
Reciever & 0.5095 & 0.6162 & 0.524 & 0.4797 & 0.5054 \\
Signal Pro. & 10.05 & 15.45 & 13.79 & \textbf{9.308} & 9.62 \\
ML Thread & 10.91 & 15.91 & 14.82 & 12.46 & \textbf{10.86} \\
\hline
ML inference$^*$ & 1.96 & 2.51 & 2.09 & 2.11 &  2.12 \\
\hline
\end{tabular}
}
\caption{T-PRIME LG pipeline performance for each block showing the \textbf{lowest latency} and \emph{lowest power} using different power profiles and ML inference optimization. The last line reports average inference times of T-PRIME LG for individual inference operations within the ML Thread. }
\label{tab: pipeline performance}
\end{table}



%We wrote a classification pipeline in Python to achieve the goal of real time protocol classification illustrated in Fig. \ref{Fig: system overview}. This pipeline consists of three primary functions that can run in parallel: receiver, signal processing, and ML inference. There are two thread safe FIFO queues, \texttt{q1} between the receiver and signal processing threads and \texttt{q2} between the signal processing and ML inference threads. This pipeline accepts several flags at run time to adjust several parameters including: center frequency, which ML model to use, and if various optimization options should be enabled. Building each of these functions as separate threads provides two main advantages. First, it allows us to parallelize our flow, removing concurrent dependencies and reducing the delay between making new predictions. Second, it allows us to modify or improve specific functions individually without having to make any changes to the other functions.




% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=0.9\linewidth]{main_python.png}
%     \caption{Pipeline diagram.  {\color{red} TODO: separate this in 2 figs: 1) pipeline goes in architecture overview, 2) UI goes in separate demo figure}}
%     \label{Fig: pipeline}
% \end{figure}

\noindent $\bullet$ \textbf{Receiver thread:} The data buffer in the receiver thread presented a crucial I/O constraint that required careful engineering. A large buffer ensured enough samples for our model, but caused frequent buffer overflows, adding over 1s to reset the connection. On the other hand, a small buffer could lead to insufficient data for the ML model, requiring multiple reads of the buffer. Thus, we designed the buffer to hold a specific number of complex samples based on the ML model used. For the LG Transformer, we configured the buffer to capture 12,900 complex samples.

%We found the data buffer in the receiver thread to be a key I/O constraint that required careful engineering. If we made the buffer very large, we are guaranteed enough samples for our model. However, do to I/O constraints this leads to frequent buffer overflow at between the SDR and the Jetson SOM. These buffer overflow can add over 1s to the timeline to reset the connection between the SDR and SOM. On the other hand, if we set the reciever data buffer too small, we may not have enough samples to feed to the ML model, resulting in multiple reads of the buffer before we have sufficient data. Therefore, we designed the buffer to hold a specific number of complex samples based on the ML model used. For the large Transformer, we configure the buffer to capture 12,900 complex samples.

\noindent $\bullet$ \textbf{Signal processing thread:} Understanding the effects of the low pass filter and re-sampling is crucial for this block. To down-sample from 31.25MHz to 20MHz, we perform rational re-sampling with a factor of $\frac{16}{25}$. For our LG Transformer trained with a 20MHz bandwidth, we need 8,192 complex samples, so the input size should be $8,192\times \frac{25}{16} = 12,800$. However, in practice, the output of this thread is slightly less than the required 8,192 samples. After empirical testing, we found that providing 12,900 complex samples as input gives the correct output size. This highlights both the complexity of deployed systems and the necessity for variable length inputs to the ML model.

%The key for this block is understanding the effects of the low pass filter and re-sampling. To down-sample from 31.25MHz to 20MHz we perform rational re-sampling with a factor of $\frac{16}{25}$. For our LG Transformer trained with a 20MHz bandwidth we need 8,192 complex samples so the input size should be $8,192\times \frac{25}{16} = 12,800$. However, in practice the output of this thread is less than the needed 8,192 samples. Instead we empirically determined we need 12,900 complex samples as the input to this block to give the correct output size. This issue highlights both the complexity of deployed systems and the need for variable length inputs to the ML model.


\noindent $\bullet$ \textbf{ML inference thread:} The key optimization for this thread was moving from PyTorch to TensorRT. The vast performance gains in the ML thread for TensorRT model shown in Table \ref{tab: pipeline performance}, without any loss of accuracy, highlight the importance of using well designed functional blocks which enable optimization of one function without making any changes to the others. 

\noindent $\bullet$ \textbf{Queue length management for real-time inference:}The above pipeline offers efficient use of computing resources, flexibility in optimizing each function, and reduced latency. However, it also presents potential bottlenecks with I/O and buffer management. To maintain low end-to-end latency, optimizing the queue length between blocks is crucial.
Long queues guarantee input availability for each function, maximizing parallelization gains and prediction rate. However, it significantly increases latency from signal reception to prediction. On the other hand, very short queues may lead to idle time, reducing parallelization efficiency and prediction rate.
Our pipeline's progressive processing times allow us to set short queues without starving any processes. However, jitters in processing time, IO blocks, and hardware limitations occasionally impact processing times dramatically. We found that setting both \texttt{q1} and \texttt{q2} to a length of 2 minimized end-to-end delay while ensuring no thread was starved. 


\subsubsection{Real-Time Deployment Results}

%\begin{figure}[tb]
%    \centering
%    \includegraphics[width=.8\linewidth]{figures/live_test.pdf}
%    \caption{T-PRIRME real-time prediction results in two new environments never seen during training.}
%    \label{Fig: real time results}
%\end{figure}

\begin{figure}
     \centering
     \begin{subfigure}[b]{0.22\textwidth}
        \centering
        \hbox{\hspace{0em} \includegraphics[width=4.1cm]{figures/live_rmD.pdf}}
        \caption{RM\_D.}
        \label{fig:RM_D}
     \end{subfigure}
     ~
     \begin{subfigure}[b]{0.22\textwidth}
        \centering
        \hbox{\hspace{0em} \includegraphics[width=4.1cm]{figures/live_rmE.pdf}}
        \caption{RM\_E.}
        \label{fig:RM_E}
     \end{subfigure}
     
        \caption{T-PRIME real-time prediction results in two new environments, RM\_D and RM\_E, never seen during training.}
        \label{Fig: real time results}
\end{figure}

Fig. \ref{Fig: real time results} shows the confusion matrix for our Real-Time evaluation where we achieve an incredible 96.7\% overall accuracy. From the confusion matrix, we see lowest accuracy is for the noise. However, given that other WiFi transmitters are operating in the area, some of the incorrect classifications for noise may in fact be correctly identifying other transmissions. Regardless, it is clear that T-PRIME has excellent accuracy in real-time predictions, even in environments it has never been exposed to during training.

%While the above pipeline allows for more efficient use of computing resources, more flexibility in optimizing each function, and reduced latency, it also introduces potential bottlenecks with I/O and buffer management. %For any real time application pipeline that conducts parallel processing, it is important to understand the average time each thread takes to process the data and to optimize the queue length between each function.  We found these times vary greatly depending on the power profile used on the NVIDIA Jetson TX2 and the version of our ML Inference thread as highlighted in Table \ref{tab: pipeline performance}. %For the highest performance settings, the Receiver thread takes 0.41 \unit{\milli\second}, the Signal Processing thread takes 9.6 \unit{\milli\second}, and the ML Inference thread takes 11 \unit{\milli\second}. 
%Optimizing the queue length between blocks is essential to maintain low end-to-end latency of a system. If the queues are very long, it guarantees each function will always have input available and maximize the gains from parallelization. While this may increase the rate at which our system makes predictions, it will also add significant latency from when the signal was actually received to when a prediction is made. If the queues are very short, there may be times when one function is waiting on data from another and cannot perform any useful work. This will reduce end-to-end latency but will also reduce the efficiency of the parallelization and the prediction rate. Because each block in our pipeline takes longer than the previous, we can keep our queues very short without worrying about starving any processes. On the other hand, jitters in the processing time, IO blocks, and hardware limitations in the receiver occasionally change the processing times dramatically. We found that setting both \texttt{q1} and \texttt{q2} to a length of 2 minimized the end to end delay while ensuring no thread was starved. 

\subsubsection{Discussion and Insights from Real-time Inference} Our implementation and testing of T-PRIME on the AIR-T device for real-time protocol classification have yielded valuable insights applicable to other AI/ML-enabled edge device classification tasks. Utilizing integrated SOM edge devices significantly reduces latencies and complexities often encountered in SDR-based systems. Parallelization plays a crucial role in increasing the prediction rate. Designing key functions as separate threads allows for more efficient resource utilization and ease of optimization for each function. Understanding I/O points and buffer management is essential for real-time systems.
%, although SOM devices generally mitigate these concerns. 
The ML Inference thread is the most resource-intensive, and optimizing this task offers significant performance gains. %in terms of latency and energy efficiency.

%Our complete implementation and thorough testing of T-PRIME on the AIR-T for real-time protocol classification have generated several take-aways that can benefit other AI/ML enabled edge device classification tasks. Utilizing integrated SOM edge devices greatly reduces latencies and complexities typically found in SDR based systems.  Parallelization is critical towards increasing the rate of predictions. Understanding the key functions and designing them as separate threads enables more efficient use of resources overall and ease of optimization for each particular function. Understanding all the I/O points and buffer management is critical for real time systems. While SOM devices generally reduce this, there are still potential friction points between various components.  The ML Inference thread is the most resource intensive. Focusing efforts on optimizing this task provide the largest performance gains in terms of latency and energy efficiency. 


%A summary of the fastest and most efficient power profiles using the baseline PyTorch and the optimized TensorRT pipeline is shown in Table \ref{tab: pipeline performance}. When configured for maximum performance, the AIR-TPC system makes a new prediction every  11 \unit{\milli\second} or 91 predictions per second. Our pipeline has an average end to end delay of 21 \unit{\milli\second}, with a maximum delay due to queuing and processing of 41 \unit{\milli\second}. 




%To better visualize the real-time inference of our system, we also created an user-friendly GUI that displays each classification as it is made. Additionally, the GUI provides an historical perspective by displaying the previous 300 predictions as a color coded time bar. This GUI can be deployed on the AIR-T device or on a remote device with network connectivity to the AIR-T. It regularly retrieves the text file with classification labels, reads the timestamps, and updates the displaya with any labels it has not yet seen.

\section{Conclusion and future work}

T-PRIME achieves near-perfect classification accuracy for 4 different WiFi protocols, outperforming legacy methods in challenging conditions. %This success demonstrates the capability of AI/ML-enabled edge devices for real-time WiFi protocol detection. 
T-PRIME proves superior to existing state of the art ML models at protocol detection, especially with low SNR and overlapping signals. While our current architecture employs fixed-length inputs, Transformers excel with variable length inputs, as shown by successful NLP models like ChatGPT. In the future, we will adapt our ML block to accommodate variable length inputs%, optimizing for accuracy and prediction speed. 
As part of our real-time implementation, we identified different  bottlenecks and offered insights for solutions, which can benefit other AI/ML-based classification systems running on resource-constrained edge devices.  %Accurate protocol identification is a crucial step for effective spectrum sharing and cognitive radios, allowing intelligent systems to optimize transmission parameters. T-PRIME outlines the path towards achieving these goals.
{\color{black} Finally, we provide public access to our code and datasets at \cite{tprime_github}.}

{\color{black} \section{Acknowledgment}
This work was funded by the Defence Science and Technology Laboratory (DSTL), a part of the UK Ministry of Defence.}


%T-PRIME achieves near perfect classification accuracy between 4 different WiFi protocols under conditions where legacy methods fail. This remarkable performance proves that AI/ML enabled edge devices can perform WiFi protocol detection in real time. We show that Transformer models are able to use IQ data directly as inputs and greatly outperform other ML models such as CNNs. Our current architecture uses a fixed length input to the Transformer, but Transformers work very well with variable length inputs, as demonstrated by the success of ChatGPT and other large NLP models. In the future, we will adapt the ML block of our pipeline to use variable length inputs. This will enable further optimization between accuracy (longer inputs) and speed of prediction (shorter inputs). 

%The T-PRIME pipeline solves several issues typically encountered in SDR based systems.  

%By understanding the key bottlenecks and engineering discrete functions that run in parallel, we provide a modular template that can be incrementally updated. These lessons can be applied to other AI/ML based classification systems that need to run on resource constrained edge devices. %In the future, we plan on expanding the ML thread to perform a wider range of detection tasks. This is particularly important as the demand for new waveforms and protocols continues to increase. 

%The first essential step to effective spectrum sharing and cognitive radios is being able to identify and understand active transmitters. Accurately identifying which protocols are in use allows intelligent systems to optimize their own transmission parameters. T-PRIME provides an outline and the first steps toward achieving these goals.


%\section*{Acknowledgment}
%This article is based upon work partially supported by XXX under grants YYY.

